Stochastic Games for Interactive Manipulation Domains

As robots become more prevalent, the complexity of robot-robot, robot-human, and robot-environment interactions increases. In these interactions, a robot needs to consider not only the effects of its own actions, but also the effects of other agents' actions and the possible interactions between agents. Previous works have considered reactive synthesis, where the human/environment is modeled as a deterministic, adversarial agent; as well as probabilistic synthesis, where the human/environment is modeled via a Markov chain. While they provide strong theoretical frameworks, there are still many aspects of human-robot interaction that cannot be fully expressed and many assumptions that must be made in each model. In this work, we propose stochastic games as a general model for human-robot interaction, which subsumes the expressivity of all previous representations. In addition, it allows us to make fewer modeling assumptions and leads to more natural and powerful models of interaction. We introduce the semantics of this abstraction and show how existing tools can be utilized to synthesize strategies to achieve complex tasks with guarantees. Further, we discuss the current computational limitations and improve the scalability by two orders of magnitude by a new way of constructing models for PRISM-games.

==> macros.tex <==
%auto-ignore
\newcommand{\ltl}{\textsc{ltl}\xspace}
\newcommand{\ltlf}{$\textsc{ltl}_f$\xspace}
\newcommand{\mdp}{\textsc{mdp}\xspace}
\newcommand{\mdps}{\textsc{mdp}s\xspace}
\newcommand{\pddl}{\textsc{pddl}\xspace}

\newcommand{\ltlphi}{\varphi}
\newcommand{\ltlfphi}{\phi}
\newcommand{\M}{\mathcal{M}}
\newcommand{\term}{\text{term}}
\newcommand{\init}{\text{init}}
\newcommand{\A}{\mathcal{A}}
\renewcommand{\L}{L}
\newcommand{\Act}{A}
\newcommand{\mypath}{w}
\newcommand{\trace}{\rho}
\newcommand{\mdpmanip}{$\mdp_{\text{manip}}$\xspace}


% New Pmax and Pmin poerators
\DeclareMathOperator*{\Pmax}{Pmax}
\DeclareMathOperator*{\Pmin}{Pmin}

% Theorems


%\newtheorem{definition}{Definition}
%\newtheorem{problem}{Problem}

\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}
\renewcommand\qedsymbol{\newline$\square$}
\newtheoremstyle{main}
                {1em}                                                % space above
                {1em}                                              % space below
                % {\hangindent=0.5em\normalfont}                                        % bodyfont
                {\normalfont}                                        % bodyfont
                {0pt}                                                % indent
                {\scshape}                                           % head font
                {\\*}                                                % head punctuation
                {2pt}                                                % head space
                {\thmname{#1}\thmnumber{ #2}: \thmnote{\itshape #3}} % head spec
                
% \theoremstyle{main}
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{claim}{Claim}
\newtheorem{problem}{Problem}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}

\newcommand{\ml}[1]{\todo[color=blue!20,size=\small,inline]{ML: #1}}
% \newcommand{\ml}[1]{\textcolor{blue}{[ML: #1]}}
% \newcommand{\aw}[1]{\textcolor{red}{[AW: #1]}}
\newcommand{\aw}[1]{\todo[color=green!25,size=\small,inline]{AW: #1}}
% \newcommand{\zk}[1]{\textcolor{green}{[ZK: #1]}}
\newcommand{\mv}[1]{\todo[color=red!25,size=\small,inline]{MV: #1}}
\newcommand{\qh}[1]{{\color{orange}[QH: #1]}}

\newcommand{\mutoref}[1]{\mbox{\autoref{#1}}}
\newcommand{\km}[1]{\textcolor{blue}{#1}}


\newcommand{\placetextbox}[3]{% \placetextbox{<horizontal pos>}{<vertical pos>}{<stuff>}
  \setbox0=\hbox{#3}% Put <stuff> in a box
  \AddToShipoutPictureFG*{% Add <stuff> to current page foreground
    \put(\LenToUnit{#1\paperwidth},\LenToUnit{#2\paperheight}){\vtop{{\null}\makebox[0pt][c]{#3}}}%
  }%
}%

\newif\ificra
\icratrue  % uncomment to see the ICRA21 version
\icrafalse
\ificra
\fi

% NOTE: Arxiv prefers idpdf pacakage - See https://info.arxiv.org/help/submit_tex.html Considerations for PDFLaTeX submissions Submission section
% Define new If statement. Refer to https://handyfloss.net/2007.08/latex-programming-how-to-implement-conditionals/ for more info on syntax
\newif\ifarxiv
\arxivtrue  % uncomment to see the Arxiv version
% \arxivfalse
\ifarxiv
\fi

==> miscellaneous/discussion_points.tex <==

\section{Motivating Examples}
In \cite{he2019efficient}, human-robot collaboration is addressed by assuming the human is adversarial. The robot must compute a policy that guarantees completion regardless of the human policy. In \cite{wells2019ltlf}, human-robot collaboration is addressed by assuming the human is probabilistic. The robot computes a policy based on the expected human actions.

The first approach suffers from being (1) overly pessimistic: many problems cannot be solved with this assumption, (2) requiring a limit on human actions: no (interesting) problems can be solved if the human has unlimited moves and (3) not allowing stochasticity: the effects of robot (and possibly human) actions are frequently stochastic.

The second approach suffers from (1) forcing stochasticity: some human behaviors cannot be represented stochastically (2) offering an unintuitive termination criteria: the game ends once a satisfying prefix is reached.

In reality, we would like to combine the behaviors of both systems. Treating the human as adversarial makes sense if (1) the human is adversarial or (2) we have insufficient information about human behaviors, but we want strong guarantees regardless. Treating the human as stochastic makes sense if we have reasonably accurate expectations of the human and we care about the expected-case performance. Stochastic robot behavior is often quite realistic.

For these reasons, we would like to combine the expressivity of \cite{he2019efficient} and \cite{wells2019ltlf} into a stochastic game. Compared to \cite{wells2019ltlf}, this allows us to express human intentions and a more intuitive stopping criteria. Consider two examples:

\subsection{Termination example}
Consider a robot tasked with cleaning a room. The room has a human operator who can move objects, but is guaranteed to eventually leave. In \cite{wells2019ltlf}, we consider the room cleaned if all objects are at their ``final'' locations, even if the human is about to move an object. Instead, we would like the robot to tidy the room until the human leaves, then finish the game once all objects are placed in their ``final'' locations and the human is gone. Here the game is terminated by the human and robot ``agreeing'' (the human by leaving and the robot by terminating).

\subsection{Human intentions}
Consider a human who wishes to build a tall tower in one of two locations, chosen with equal probability at the outset of the run. Modeling human behavior with a probability distribution over (short) sequences of actions cannot express longer-term behaviors than the length of the longest sequence, given the Markov assumption holds.

Instead, it is more reasonable to think about a human policy with some stochastic action(s) (choosing the location for the tower) and other actions chosen according to an ``intention.''


\subsection{Other examples}
In general, we can use any example where using a human probability distribution doesn't make sense, but where we still want to have stochastic effects. I think you can ``layer'' random and strategic human moves, to describe a wide variety of scenarios:

Driving where we have a set of likely actions for cars to take, but also need to reason over worst-case occurrences.
Construction where we don't know what the human is building, but have some probability distribution.
etc.


\subsection{Limiting human behaviors}
In several examples, we would like to limit the human to some behavior: e.g., finite executions. In many cases, I think we can take the logical implication $(\neg human\_behavior \vee robot\_goal)$. For some cases, e.g., termination, this may not work well:

 $(G \neg h\_term \vee r\_win)$
 
 Here, $G \neg h\_term$ is infinite trace.




\section{Modeling Discussion}
We face several questions in modeling the problem:

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|}
        \hline
        concurrent game & turn-based game \\
        \hline
        X & Better understood \\
        \hline
        More expressive & X \\
        \hline
        No path formulas in PRISM & No path formulas in PRISM\\
        \hline
        LTLf seems obvious? & LTLf theory exists \\
        \hline
    \end{tabular}
    \caption{Concurrent vs turn-based games}
    \label{tab:my_label}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        Satisfying prefix & negotiated terminal state & non-zero human term \\
        \hline
        Similar to MDPs & X & X \\
        \hline
        least intuitive & tie? & tie? \\
        \hline
        X & Most expressive? & X \\
        \hline
        supported & no path formula & supported\\
        \hline
    \end{tabular}
    \caption{How to define termination}
    \label{tab:my_label}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        Instantaneous, discrete state change & cost remaining & ? \\
        \hline
        Already used & X & X \\
        \hline
        what if human doesn't interrupt? & X? & ?  \\
        \hline
        X & infinite state space? & ? \\
        \hline
        more expressive human & tie? & ? \\
        \hline
    \end{tabular}
    \caption{How to handle interruptions}
    \label{tab:my_label}
\end{table}

In the ICRA paper, we assume human probability distributions are Markovian w.r.t. the state space of our MDP. I think this was overly limiting. Allowing human choices should avoid the issue?

Desired behavior for interruption:
If the human moves, the robot should cede priority to the human.
The robot should reevaluate its next move every time the human moves.
The robot should not repeatedly wait for the human to move. (I think a weakness from ICRA paper). Ideally the robot should succeed, even when the stochastic model is inaccurate.


==> root.tex <==
%auto-ignore
\input{imports}

% any commands that I will want to use a lot
\input{macros.tex}

\input{title.tex}

% body of document
\begin{document}

\ifarxiv
\placetextbox{0.5}{0.95}{To appear at the 2024 IEEE International Conference on Robotics and Automation (ICRA), May 2024.}
\fi

\maketitle
\thispagestyle{plain}
\pagestyle{plain}

\input{sections/abstract}
\input{sections/introduction}
% \input{sections/preliminaries}
\input{sections/problem_setup}
\input{sections/modeling}
\input{sections/synthesis}
\input{sections/results}
\input{sections/conclusion}

% \section*{ACKNOWLEDGMENTS}
% Work by KM and ML are supported by NASA through grant \#80NSSC21K1031.
% Work by LEK and MYV are supported by NSF 1830549. Work by AMW supported by NASA 80NSSC17K0162. 
% We would like to thank the authors of PRISM, especially Dave Parker for their excellent tool and for their help in modifying it to import stochastic games. 
% We would like to thank Karan Muvala and especially Peter Amorese for their help with the Panda robot.

% \clearpage{}
\bibliographystyle{IEEEtran}
\bibliography{IEEEabrv,refs}

\end{document}


==> sections/iros_modeling.tex <==
\section{Modeling}
\label{sec:modeling}

% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%  Stochastic Game        & Robotics Domain        \\
%  \hline
%  Discrete states + actions        & Continuous states + actions      \\
%  Turn-based             & Free-form actions      \\
%  Limited human model  & Flexible human capabilities \\
%  Specified termination  & Unconstrained termination     \\
%  \hline
% \end{tabular}
% \caption{Primary challenges to modeling human-robot manipulation as a stochastic game. \km{``Arent Limited human model" and ``Specified termination" limitation of reactive and probabilistic models that we are trying to relax using SMGs?}}
% \label{table:modeling_challenges}
% \end{center}
% \end{table}

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{0.3\columnwidth}
%         \includegraphics[width=\textwidth]{figs/abs_init_state}%
%         % \caption{}
%         \label{fig:start_state}
%     \end{subfigure}
%     \qquad \quad
%     \begin{subfigure}{0.3\columnwidth}
%         \includegraphics[width=\textwidth]{figs/abstract_robot_state}
%         % \caption{}
%         \label{fig:robot_act}
%     \end{subfigure}
%         \qquad \quad
%     \begin{subfigure}{0.3\columnwidth}
%         \includegraphics[width=\textwidth]{figs/abstract_human_state}
%         % \caption{}
%         \label{fig:human_act}
%     \end{subfigure}
%     \caption{Manipulation domain: (left) the initial state. (right) the result of a robot ``pick'' action. (center) the result of an attempted robot ``place'' action that was interrupted by the human.}
%     \label{fig:abs_manip}
% \end{figure}

Now we discuss how to model \autoref{def:manip_domain_abstraction} as a stochastic game. There are four main challenges, listed in \autoref{table:modeling_challenges}. We discuss each in turn.



\subsection{Discretizing States and Actions}
To discretize states and actions, we follow prior works in reactive or probablistic synthesis for robot manipulation \cite{He:RAL:2018, he2019efficient, wells2021probabilistic} \km{Stating it this way suggests that there is no contribution from this paper.}. States are discretized by specifying a finite number of ``regions of interest.'' These must \km{no must} include the robot gripper and any regions needed to satisfy predicates in the specification \km{``predicates" is used for the first time.}. All regions not specified are grouped together as the ``Else'' region (see \autoref{fig:toy_example}). This gives us $S$ and $s_o$ from \autoref{def:stochastic_game}. If applicable, costs can be associated with moving from one region to another to model, e.g., traversal time. \cite{He:RAL:2018} gives an automated method for constructing such abstractions.

The way actions are discretized varies for deterministic vs stochastic actions. For deterministic actions, we follow PDDL manipulation domains \cite{pddl} for both the human and the robot. Issues arising from simultaneous or interrupted actions will be discussed in \autoref{sec:allocating_turns}.

% \begin{example}
%     For a purely strategic human, the manipulation domain \km{which one? SMG or Def. 1 Abstraction? or MDP?} becomes a deterministic transition system. \km{Not clear to me}
    
%     \begin{figure}[h]
%         \vspace{0em}
%             \centering
%             \scalebox{0.94}{
%             \begin{tikzpicture}[auto,node distance=2.5cm,on grid,line width=0.4mm]
%                 \tikzstyle{round}=[thick,draw=black,circle]
        
%                 % \node[state, label={\footnotesize $\emptyset$}] (s0) {$\langle 1,2,3 \rangle$};
%                 \node[state,inner sep=1pt,minimum size=0pt] (s0) {\includegraphics[width=11mm]{figs/arch_init}};
%                 \node[state,inner sep=1pt,minimum size=0pt] (s1) [right=of s0] {\includegraphics[width=11mm]{figs/arch_grasped}};
%                 \node[state,inner sep=1pt,minimum size=0pt] (s2) [below=1cm of $(s0)!0.5!(s1)$] {\includegraphics[width=11mm]{figs/arch_other}};
%                 \node[state,accepting,inner sep=1pt,minimum size=0pt] (s3) [right=of s1] {\includegraphics[width=11mm]{figs/arch_final}};		
        
%                 \path[->] 	(s0) edge node {} (s1)
%                             (s0) edge node {} (s2);
%                 \path[->] 	(s1) edge [bend right=45] node [above] {} (s0)
%                             (s1) edge node [above] {} (s3);
%                 \path[->] 	(s2) edge [bend left=45] node [below] {} (s0);
                            
%             \end{tikzpicture}
%             }
%             \caption{Example portion of abstraction of manipulation domain for a deterministic pick-and-place domain. 
%             % The state-space is explained in \autoref{fig:toy_example}.
%             }
%             \label{fig:example_deterministic}
%     \end{figure}
% \end{example}

For stochastic actions, we follow \cite{wells2021probabilistic}. To handle simultaneous actions, we build a combined probability distribution from the probabilities of effects of robot actions and human actions (if applicable). Stochastic human actions are not strategic, but a strategic human may choose between different stochastic actions. When modeling stochastic human actions, we allow several actions to be ``chained'' into one turn as in \cite{wells2021probabilistic}. Note that the human cannot alter the robot's end-effector \autoref{fig:abs_manip}:

% \begin{example}
% \begin{figure}[h]
%     \vspace{-1em}
%     \label{ex:example_mdp_human}
%         \centering
%         \begin{tikzpicture}[auto,node distance=3cm,on grid,line width=0.4mm]
%           \tikzstyle{round}=[thick,draw=black,circle]
    
%             \node[state,inner sep=1pt,minimum size=0pt] (s0) {\includegraphics[width=13mm]{figs/arch_init}};
%             \node[state,accepting,inner sep=1pt,minimum size=0pt] (s1) [right=3.5cm of s0] {\includegraphics[width=13mm]{figs/arch_final}};
%             \node[state,inner sep=1pt,minimum size=0pt] (s2) [below=2.1cm of s0] {\includegraphics[width=13mm]{figs/arch_red_empty}};
%             \node[state,inner sep=1pt,minimum size=0pt] (s3) [below=2.1cm of s1] {\includegraphics[width=13mm]{figs/arch_empty_yellow}};		

%             \node[state,inner sep=1pt,minimum size=0pt] (s4) [above=2.1cm of s0] {\includegraphics[width=13mm]{figs/arch_another}};
%             \node[state,inner sep=1pt,minimum size=0pt] (s5) [above=2.1cm of s1] {\includegraphics[width=13mm]{figs/arch_yellow_red}};
%             \node[draw=none,fill=none, right=1.5cm of s4] {\Large\dots};
    
%             \path[->] 	(s0) edge [in=180,out=0,pos=0.8] node [above] {\footnotesize 0.15} (s1)
%                         (s0) edge [in=55,out=0,pos=0.8] node [left=1mm] {\footnotesize 0.15} (s2)
%                         (s0) edge [in=125,out=0,pos=0.8] node [left=1mm] {\footnotesize 0.15} (s3)
%                         (s0) edge [in=12,out=2,loop,pos=0.9] node [above=1mm] {\footnotesize 0.4} ()
%                         (s0) edge [in=340,out=0,pos=1] node [above=0.25mm, right=1mm] {\footnotesize 0.03} (s4)
%                         (s0) edge [in=195,out=0,pos=0.9] node [below=1mm] {\footnotesize 0.03} (s5);
%             % \path[->] 	(s1) edge node [above] {\footnotesize 0.9} (s0)
%             %             (s1) edge [in=195,out=180,loop,pos=0.9] node [below=1mm] {\footnotesize 0.1} ()
%             %             (s1) edge node [above,pos=0.7] {\footnotesize 0.9} (s3)
%             %             (s1) edge [in=15,out=0,loop,pos=0.9] node [above=1mm] {\footnotesize 0.1} ();
%             % \path[->] 	(s2) edge [bend right=30,pos=0.9] node [right=1mm] {\footnotesize 0.9} (s0)
%             %             (s2) edge [in=110,out=100,loop,pos=0.9] node [left=0.25mm] {\footnotesize 0.1} ();
%             %% loop for the action
%             % \path pic[draw, angle radius=7mm,"\vphantom{g} \footnotesize{$a_1$}",angle eccentricity=1.3] {angle = s2--s0--s1};
            
%         \end{tikzpicture}
%         \caption{Example portion of an MDP encoding human actions. In the top row, the human has moved two blocks. In the remaining states, the human has moved one or no blocks.}
%         \label{fig:examplemdp}
%     \vspace{-1em}
% \end{figure}
% The human has probabilities for moving none, one or several of the blocks in \autoref{fig:examplemdp}. The robot can concurrently attempt to move blocks, deferring to the human in the case of conflict. The result is a system with many possible transitions between states, where each transition can encode several block motions. For example in the top left, the robot may have tried to grasp the blue block, and have been overridden by the human. The human moved the yellow and then the blue block in one transition. \km{The figure and the Example is not clear to me,}
% \end{example}

This give us \km{Probabilistic Transition Relation} $T$ (\autoref{def:stochastic_game}). For a discussion of how various ``chaining'' actions affects scalability, see \cite{wells2021probabilistic}.

% \subsection{2.5-player game}
% In our model, we have two strategic agents as well as stochastic effects caused by ``nature.'' The stochastic effects can apply to both, one or neither player. When stochastic effects apply to at least one player, we have a 2.5-player game (one system player, one environment player and the half-player of ``nature'').

% For the strategic players, we follow the models of prior works \cite{he2019efficient}. The robotic agent follows a standard pick-place domain, which typically can be encoded in 
% PDDL. The human player has the same abilities, but is assumed to move relatively quickly compared to the robot. Additionally, as a modeling assumption, we do not allow the human to hold onto an object (as in prior works \cite{he2019efficient}). Thus we model the robot's gripper but no human gripper.

\subsection{Modelling Manipulation as a Turn-Based Game}
\label{sec:allocating_turns}
In free-form human-robot interaction, there is no notion of a ``turn.'' Tools such as Prism Games \cite{kwiatkowska2020prism} can handle concurrent rather than turn-based games, but with greater computational cost \km{cite}. Because scalability is already a significant challenge, we stick to turn-based games. 

We essentially need to answer two questions: Whose turn is it? ($C$ from \autoref{def:stochastic_game}) And what can an agent do in this (one) turn? ($A$ from \autoref{def:stochastic_game})

Following prior work, we assume the human can move faster than the robot, leading to multiple human moves per robot move. To maximize human flexibility, we always allow the human to act. Because we do not want the robot to waste time, the robot always attempts to act. As in \cite{He:IROS:2017}, we assume certain robot actions are ``atomic'' while giving the human actions priority over all non-atomic actions. Here, as in previous work, the atomic robot actions are grasp and place (not including the transit or transfer preceding the opening / closing of the gripper). We try to grant the human greater flexibility than the robot in our models. E.g., by allowing multiple human actions in quick succession or by giving the human priority over the robot \autoref{fig:toy_example}. \km{Up Until this point, everything seems to be done in prior work.}

At each state, the robot consults its policy to find the optimal action, then attempts to perform that action. If the state updates before the robot completes its action, it considers the human turn finished and again consults its policy to find the optimal action in the new state. If the human acts again, the robot proceeds in the same way. \km{The first part is a little ambiguous.} The human has exceeded its action limits (see below), but so long as the resulting state is included in the robot policy, the robot will still have an optimal response (under the modeling assumptions) for the new state.


\subsection{Weakening Assumptions (Limits) on Human Behavior}

Previous works \cite{He:IROS:2017, He:RAL:2018, he2019efficient} had to include additional restrictions such as limiting the number of actions or the rate of actions. A limit \emph{k} is placed on the total number of human actions to ensure the specification is realizable. This limit is unintuitive and somewhat unrealistic. For example, suppose the model assumes the human  makes at most 30 actions ($k = 30$). Then during execution, once the robot observes the $30^{th}$ action, it will act as though the human will no longer interfere. Unfortunately, unless there is some external reason for this limit, the robot should arguably assume the human is \emph{more} likely to interfere because it has observed this happen $30$ times already. \km{Add discussion on how this can be implemented using games but the stochasticity associated with each agent can not be captured like a robot failing to grasp a small object.}

We generalize this as a \emph{ratio} of human and robot actions. For example we could allow 1 human action for every 2 robot actions (denoted by $2:1$). 
\km{Mention that a winning strategy may not exist.} We implement this using counters that reset every time the game changes control from one player to another. $C$ and $A$ (\autoref{def:stochastic_game}) are defined such that no motion can be made once this threshold is exceeded. Note a player cannot ``skip'' turns now in order to take more consecutive turns later. \km{Remove this line.} This means, $4:2$ is not necessarily the same as $2:1$. \km{how is this a natural weakening of the limit? Why does this make sense for real-world applications? This weakness is unintuitive!}

We also present a model using a probability of handing control from one player to another \km{This is not true. We mention probability of human termination which is more expressive for the human agent and also scalable. The state space of the SMG using counters will blow up as you increase the ratio.}. This implies a probabilistic limit, but avoids setting a hard limit on action for either player. For example, instead of limiting the human to $k=30$ actions, we could give the human a probability of stopping after each action $p_k = 1/30$. In our experiments, we find this more flexible model leads to only minor extra computational cost.

\subsection{Termination}
Finally, we have to define some notion of who wins the game \km{This is the first time ``winning the game" term is introduced. We need to elaborate in the above section that winning associates with reaching an accepting state}. In previous works, this was done by accepting finite prefixes. This can be uninuitive, for example a robot asked to clean the room will stop once the room is cleaned, even if the human is approaching some object to displace it. In our new model, we would like to allow the human and robot to ``negotiate'' termination so that the robot only considers the task complete when the human agrees. \km{It does not make sense to use/discuss LTLf if we are reasoning over possibly infinite traces.}

For a given \ltlf\ specification (e.g., eventually construct some object), synthesis reduces to solving a stochastic game for a reachability objective that corresponds to reaching the accepting state of the deterministic finite automata expressed by the \ltlf\ specification. Thus $L$ \km{I Think this is $\mathcal{L}$ from \ltlf semantics definition.} (\autoref{def:stochastic_game}) is defined by reaching this set of states.


A partial stochastic game for our manipulation domain is shown in \autoref{fig:stochastic_game}.

\begin{figure}[h!]
    \label{ex:example_stochastic_game}
        \centering
        \begin{tikzpicture}[auto,node distance=3cm,on grid,line width=0.4mm]
        %   \tikzstyle{round}=[thick,draw=black,circle]
          
    
            \node[circle,draw,state,inner sep=1pt,minimum size=0pt] (s0) {\includegraphics[width=13mm]{figs/arch_init}};
            \node[rectangle,draw,inner sep=4pt,minimum size=0pt] (s1) [below left=of s0] {\includegraphics[width=13mm]{figs/arch_grasped}};
            \node[rectangle,draw,inner sep=4pt,minimum size=0pt] (s2) [below right= of s0] {\includegraphics[width=13mm]{figs/arch_other}};
            \node[circle,draw,state,accepting,inner sep=1pt,minimum size=0pt] (s3) [below =2.1cm of s1] {\includegraphics[width=13mm]{figs/arch_final}};
            \node[circle,draw,state,inner sep=1pt,minimum size=0pt] (s4) [below left=of s2] {\includegraphics[width=13mm]{figs/arch_other}};
            \node[circle,draw,state,inner sep=1pt,minimum size=0pt] (s5) [below right=of s2] {\includegraphics[width=13mm]{figs/arch_another}};
    
            \path[->]       (s0) edge (s1)
                            (s0) edge (s2);
            \path[->]       (s1) edge (s3);
            \path[->]       (s2) edge (s4)
                            (s2) edge (s5);
    
            % \path[->] 	(s0) edge [bend left=55] node [above] {\footnotesize 0.9} (s1)
            %             (s0) edge [bend left=55] node [below] {\footnotesize \emph{grasp blue}} (s1)
            %             (s0) edge [in=75,out=55,loop,pos=0.7] node [left=1mm] {\footnotesize 0.1} ()
            %             (s0) edge [bend right=50] node [left=1mm] {\footnotesize 0.9} (s2)
            %             (s0) edge [bend right=50] node [right=0.5mm] {\footnotesize \emph{grasp yellow}} (s2)
            %             (s0) edge [in=210,out=220,loop,pos=0.9] node [left=1mm] {\footnotesize 0.1} ();
            % \path[->] 	(s1) edge node [above,pos=0.7] {\footnotesize 0.9} (s0)
            %             (s1) edge node [below] {\footnotesize \emph{put blue}} (s0)
            %             (s1) edge [in=165,out=180,loop,pos=0.9] node [above=1mm] {\footnotesize 0.1} ()
            %             (s1) edge node [above,pos=0.7] {\footnotesize 0.9} (s3)
            %             (s1) edge node [below,pos=0.5] {\footnotesize \emph{stack blue}} (s3)
            %             (s1) edge [in=15,out=0,loop,pos=0.9] node [above=1mm] {\footnotesize 0.1} ();
            % \path[->] 	(s2) edge [bend right=45,pos=0.7] node [right=1mm] {\footnotesize 0.9} (s0)
            %             (s2) edge [bend right=45,pos=0.4] node [right=1mm] {\footnotesize \emph{put yellow}} (s0)
            %             (s2) edge [in=30,out=45,loop,pos=0.9] node [right=0.25mm] {\footnotesize 0.1} ();
    
            %% loop for the action
            % \path pic[draw, angle radius=7mm,"\vphantom{g} \footnotesize{$a_1$}",angle eccentricity=1.3] {angle = s2--s0--s1};
            
        \end{tikzpicture}
        \caption{Partial stochastic game for pick-and-place domain. Transitions can have probabilities to model stochastic effects, errors or random choices. \km{This graph is not very clear. We should illustrate stochasticity. Also, How did the Yellow object disappear from the Robot's hand? Human can move an object from the robot's end effector and we did not skip a robot turn, so this needs to be fixed.}}
        \label{fig:stochastic_game}
    \vspace{0em}
\end{figure}

The actions taken in circular states are controlled by the system and those taken in rectangular states are controlled by the environment. The same action could stochastically lead to different possible states (e.g., in the above the robot's first action could attempt to pickup a cylinder from the initial state and stochastically determine whether to grasp the yellow or the blue cylinder).

\subsection{Solving the Game}
Our \ltlf specifications can be made into reachability objectives. Then there exists an optimal memoryless, deterministic policy for each player \km{significance of being memoryless and detemrinistic?}. The game can be solved using value iteration until some convergence criteria is met \cite{chen2013automatic}. How many iterations this will take is an open question, and solving stochastic games with reachability objectives lies in the complexity class $NP \cap coNP$ \cite{condon1993algorithms}.

==> sections/iros_preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

 We begin by discussing our model of robot manipulation. Then we discuss logical specifications for these domains and stochastic models used to reason over logical specifications.

\subsection{Manipulation Domain}

As a starting point, we use a manipulation domain abstraction based off of \cite{He:RAL:2018}. 


\begin{definition}[Abstraction of a Manipulation Domain]
    \label{def:manip_domain_abstraction}
	An \emph{abstract manipulation domain} is a tuple: $G_{det}=(S, s_0, A_s, A_e, T, AP, L)$ where,
	\begin{itemize}
		\item $S$ is a finite set of states,
		\item $s_0 \in S$ is the initial state,
		\item $A_s$ is the finite set of system (robot) actions,
		\item $A_e$ is the finite set of environment (human) actions,
		\item $T : S \times (A_s \cup A_e) \mapsto S$ is the transition function,
		\item $AP$ is the set of task-related atomic propositions,
		\item $L : S \mapsto 2^{AP}$ is the labeling function that maps each state to a set of atomic propositions.
	\end{itemize}
\end{definition}

As an example, consider the abstract manipulation domain depicted in \autoref{fig:toy_example}. There are two agents, a robot and a human. Each agent can change the state of the world, albeit under some restrictions. For the robot, these restrictions follow typical PDDL pick-place domains \cite{pddl}. For example, the robot cannot pickup an object while it is supporting another object \autoref{fig:toy_example}. For the human, various assumptions are introduced to make the problem tractable \cite{he2019efficient, wells2021probabilistic}. We discuss how stochastic games allow us to relax these assumptions in \autoref{sec:modeling}.


% \begin{figure}[h]
%   \begin{center}
%     \includegraphics[width=0.3\textwidth]{figs/abs_init_state}
%   \end{center}
%   \caption{Abstract initial state}
%   \label{fig:start_state}
% \end{figure}

% \begin{figure}[h]
% 	\begin{center}
% 	  \includegraphics[width=0.3\textwidth]{figs/abstract_robot_state}
% 	\end{center}
% 	\caption{Abstract state after robot action}
% 	\label{fig:robot_act}
% \end{figure}

% \begin{figure}[h]
% 	\begin{center}
% 	  \includegraphics[width=0.3\textwidth]{figs/abstract_human_state}
% 	\end{center}
% 	\caption{Abstract state after robot tries to place the yellow object and the human interrupts}
% 	\label{fig:human_act}
% \end{figure}


Once we have a model of a manipulation domain, we next need some formal way to express properties of ``runs'' (executions) through this domain.
% As in \cite{wells2021probabilistic}, we use ``missing'' objects to denote objects in the ``Else'' region (see \autoref{fig:toy_example}).

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.25\columnwidth}
        \includegraphics[width=\textwidth]{figs/arch_locs}%
        % \caption{}
        \label{fig:toy_example_setup}
    \end{subfigure}
    \qquad \quad
    \begin{subfigure}{0.25\columnwidth}
        \includegraphics[width=\textwidth]{figs/arch_init}
        % \caption{}
        \label{fig:toy_example_initial}
    \end{subfigure}
    \vspace{-1em}
    \caption{Manipulation domain: (left) the locations of interest, where the Else location ($Loc_1$) contains all objects not otherwise shown.
    (right) Initial state with red and yellow blocks at $Loc_2$ and $Loc_3$.
    % and the blue block at $Loc_1$.
    }
    \label{fig:toy_example}
\end{figure}

\subsection{Linear Temporal Logic over Finite Traces}
Linear temporal logic (\ltl) \cite{pnueli1977temporal} is a popular formalism used to specify temporal properties over infinite horizons. In robotics, we are frequently interested in \ltl interpreted over finite execution or traces (\ltlf) \cite{de2013linear}. 

\begin{definition}[\ltlf Syntax]
	An \ltlf formula is built from a set of atomic propositions $AP$ and is closed under the Boolean connectives as well as the ``next'' operator $X$ and the ``until'' operator $U$:
	\[
		\ltlfphi ::= \top   \mid   p   \mid   (\neg \ltlfphi)   \mid   (\ltlfphi_1 \wedge \ltlfphi_2)   \mid   (X \ltlfphi)  \mid  (\ltlfphi_1 U \ltlfphi_2)
	\]
	where $p \in AP$, $\top$ is ``true'', and $\neg$ and $\wedge$ are the ``negation'' and ``and'' operators in Boolean logic respectively.
\end{definition}

\noindent
The common temporal operators ``eventually'' ($F$) and ``globally'' ($G$) are defined as: $F \, \ltlfphi = \top \, U \, \ltlfphi$ and $G \, \ltlfphi = \neg F\, \neg \ltlfphi$.

We can use \ltlf to express a property such as ``this construction task must be completed safely.''

\begin{example}[Example \ltlf specification]

Consider the \ltlf formula

$$ F\ constructed \wedge G\ \neg\ safety\_violation $$

Read ``Eventually $Constructed$ and Globally not $safety\_violation$''. This could be used to specify that the robot must finish construction in finite time and while doing so must not move to an unsafe state (a state where the robot is too close to the human).

\end{example}

% For a more thorough treatment of \ltlf, see \cite{de2013linear, de2015synthesis} or similar.

The semantics of \ltlf are defined as follows.

\begin{definition}[\ltlf Semantics]
	The semantics of an \ltlf \hspace{0.5mm}formula are defined over finite traces. A trace $\rho$ is a word in $(2^{AP})^*$. Let $|\rho|$ denote the length of trace $\rho$ and $\rho[i]$ be the $i^{th}$ symbol of $\rho$. Further, $\rho, i \models \ltlfphi$ is read as: ``the $i^{th}$ step of trace $\rho$ is a model of $\ltlfphi$.'':
	\begin{itemize}
		\item $\rho , i \models \top;$
		\item $\rho , i \models p$ iff $p \in \rho[i];$
		\item $\rho , i \models \neg \ltlfphi$ iff $\rho, i \not \models \ltlfphi;$
		\item $\rho , i \models \ltlfphi_1 \wedge \ltlfphi_2$, iff, $\rho, i \models \ltlfphi_1$ and $\rho, i \models \ltlfphi_2;$
		\item $\rho , i \models X \ltlfphi$ iff $|\rho| > i+1$ and $\rho, i+1 \models \ltlfphi;$
		\item $\rho , i \models \ltlfphi_1 U \ltlfphi_2$ iff $\exists j$ s.t. $ i \leq j < |\rho|$ and $\rho, j \models \ltlfphi_2$ and $\forall k$, $i \leq k < j$, \; $\rho, k \models \ltlfphi_1$,
	\end{itemize}
\end{definition}
Finite trace $\rho$ satisfies $\ltlfphi$, denoted by $\rho \models \ltlfphi$, if $\rho, 0 \models \ltlfphi$.
An $LTL_f$ formula $\ltlfphi$ defines a language $\mathcal{L}(\ltlfphi)$ over the alphabet $2^{AP}$. $\mathcal{L}(\ltlfphi)$ is a regular language, more specifically, $\mathcal{L(\ltlfphi)} = \{\rho \in (2^{AP})^* \mid \rho \models \ltlfphi\}$.  \km{This can be shortened to save up space.}
% (recall that \ltlf has the expressivity of star-free regular languages).



% \subsection{Probabilistic Abstraction of Manipulation Domain}
% We extend our manipulation domain abstraction $G_{prob}$ by introducing non-deterministic actions to be controlled by the environment.

% \begin{definition}[Probabilistic Abstraction of a Manipulation Domain]
% The probabilistic abstraction of a manipulation domain is a tuple: $G_{stoch\_game}=(S, s_0, A_s, A_e, T_e, AP, L, P_s, P_e)$ where $S, s_0, A_s, A_e, AP$ and $L$ are defined as in  \autoref{def:manip_domain_abstraction} and
% \begin{itemize}
% 	\item $S$ is a finite set of states,
% 	\item $s_0 \in S$ is the initial state,
% 	\item $A_s$ is the finite set of system (robot) actions,
% 	\item $A_e$ is the finite set of environment (human) actions,
% % 	\item $T : S \times (A_s \cup A_e) \mapsto S$ is the transition function,
% 	\item $T_e$ gives the result of applying human action $act_e \in A_e$ at state $s \in S$. $T_e: S \times A_e \times S \to \{0,1\}$.
% 	\item $AP$ is the set of task-related atomic propositions,
% 	\item $L : S \mapsto 2^{AP}$ is the labeling function that maps each state to a set of atomic propositions.
% 	\item $P_s$  is a probability function $P_s: S \times A_s \times S \to [0,1]$ that gives the probability distribution of effects of system (robot) actions as the probability $P_s(s_{i+1} \mid act_s, s_i)$,
% 	\item $P_e$ is a probability function $P_e: S \times A_e \to [0,1]$ that gives the probability of an environment (human) action being applied at the current state $P_e(act_e \in A_e \mid s_i)$.
% \end{itemize}
% \end{definition}

% Description.

\subsubsection{Stochastic Games}
Here, we formally define stochastic games, which we will use to model human-robot manipulation in \autoref{sec:modeling}.
\begin{definition}[Stochastic Game]
A stochastic game is a tuple $G = (S, s_0, A, T, C, AP, L)$ where $S, s_0, AP$ and $L$ are as in \autoref{def:manip_domain_abstraction} and :
\begin{itemize}
    \item $A$ is the finite set of actions \km{How is this different from $A_s$ and $A_e$. Is it not $A = A_s \cup A_e?$}
    \item $T: S \times A \times S \mapsto [0,1]$ is the probabilistic transition relation
    \item $C: S \mapsto \mathbb{N}$ designates which player controls the choice of action at each state
\end{itemize}
We say $G$ is a two-player stochastic game when $C : S \mapsto \{0,1\}$.
\label{def:stochastic_game}
\end{definition}
Intuitively, a stochastic game is similar to an MDP except that there are two (or more) independent strategic agents that take turns making choices. For more details on stochastic games, see \cite{kwiatkowska2020prism, fundberg1991game}

\begin{definition}[Path through a Stochastic Game]
A path through a stochastic game is a finite sequence of states
$\lambda : s_0, ..., s_n$
\end{definition}

\begin{definition}[Policy for a Stochastic Game]
A policy for a stochastic game is a function from a history of states and an action to a probability.
$\sigma : \lambda \times A \mapsto [0,1]$
such that for any $\lambda$, $\sum_{act \in A} \sigma(\lambda, act) = 1$
\end{definition}

For two player stochastic games with a reachability objective memoryless, deterministic strategies suffice \cite{chen2013automatic}. 


==> sections/iros_results.tex <==
\section{Results}
Stochastic games subsume the expressivity of both reactive and probabilistic synthesis, but they also bring even more challenges to scalability. We present simple benchmarks based on experiments from \cite{wells2021probabilistic}. Our experiments are available online \cite{wells2021github}. 

% We run our test using Prism-Games \cite{kwiatkowska2020prism}, an open-source tool implemented in Java. \km{Rmeove all of this. Maybe keep the Implementation improvements}. We make small modifications to remove a performance bottleneck when importing models and these changes have been submitted as a pull request to Prism. All experiments are run on a Ryzen 9 5950x and RAM limits are set for the JVM via command line arguments (see below).
% Our experiments are available online \cite{wells2021github}. 
% We have also created Docker images to aid reproducibility \cite{wells2021docker}.


\subsection{Comparison to Reactive and Probabilistic Synthesis}
\label{sec:qual_comp}
Because we are the first to present a framework for solving manipulation problems via stochastic games, there is no direct comparison point for our method. Instead, we compare to prior works for reactive or probabilistic synthesis to showcase the strengths and weaknesses of the different approaches.

\subsubsection{Reactive Synthesis}
In \cite{He:IROS:2017, He:RAL:2018, he2019efficient}, reactive synthesis is used to solve human-robot manipulation in a setting similar to our own. In these frameworks, there is no way to reason about stochastic effects of actions. Consider the problem presented in \autoref{fig:abs_manip}. We may know that each object can be grasped with a different probability of success, but if we use reactive synthesis we cannot exploit this knowledge (unless the probability is 0 or 1). Reactive synthesis considers the worst case, so any probability less than 1 will be treated as leading to failure. By modeling the problem as a stochastic game, we can gain the benefits of reactive synthesis while still favoring actions that are more likely to be successful. The downside is that stochastic games are more computationally complex to solve. Stochastic games can also be used to model a finite number of human actions without imposing a specific bound (see \autoref{table:manip_prob}).

\subsubsection{Probabilistic Synthesis}
In \cite{wells2021probabilistic}, human-robot manipulation is modeled as an MDP and solved via probabilistic synthesis. This allows us to express actions with stochastic effects, but it also requires us to model human behavior as a probability distribution. In many cases, we do not have data to support such a model. \km{mention strategic nature of human that MDP can not capture} Consider the example in \autoref{fig:abs_manip}.

\begin{figure}[h!]
  \centering
  \begin{subfigure}[b]{0.15\textwidth}
      \includegraphics[width=\textwidth]{figs/3_block}
      \caption{3 block}
  \end{subfigure}
  \hspace{2em}
  \begin{subfigure}[b]{0.15\textwidth}
      \includegraphics[width=\textwidth]{figs/4_block}
      \caption{4 block}
  \end{subfigure}
  \caption{Goals used in our experiments}
  \label{fig:experiment_scenes}
\end{figure}

\begin{example}[MDP vs Stochastic Game for Manipulation]

Consider a scenario with three blocks. In the absence of data, we can follow the model used in \cite{wells2021probabilistic} (in brief, at any state there is a $40\%$ chance the human does not act and the remaining probability is split evenly among the available actions). For our stochastic game, let us assume the human acts strategically (to bound our worst case behavior) and at every state the human has probability $0.05$ of getting bored and leaving \km{Add comment staying ``Notice how we are weakening assumptions about the human (it could be off) that game based approached do not allow "}.

For the true human model, let's assume we are completely off. The human will get bored after exactly 7 moves and until then will insist on moving the yellow block to the location nearest the human.

For the robot, assume picking up the red, yellow and blue objects succeed with probabilities $0.9,\ 0.7\ and\ 0.5$ respectively. We assume both the stochastic game and the MDP model this accurately, as we could easily ascertain these probabilities experimentally.


\begin{table}[h]
\begin{tabular}{ |c|c|c|c| } 
 \hline
                      & MDP   & Stochastic Game  & Optimal\\ 
 \hline
 Expected Cost              & 11.5 actions          & 12.4 actions    & 9.4 actions  \\ 
 \hline
\end{tabular}
\caption{Comparison of two inaccurate models, one an MDP and the other a Stochastic Game. While both models are inaccurate, the stochastic game is more robust.}
\label{table:inaccurate_models}
\vspace{-1em}
\end{table}

\end{example}

It is important to note what is happening here. The stochastic game is \emph{not a more accurate model} than the MDP. Of course, it could be, in which case the stochastic game would be even better; but here \emph{both models are inaccurate. The stochastic game is a more robust model than the MDP}.  \km{Written way too informally. Need to be more direct.}

The human in this example is not strategic. So human-robot manipulation would be optimally solved by an MDP. Obviously stochastic games are not a better way to solve MDPs on average, but they bound the worst case (as in this example). For strategic human models, Stochastic Games are accurate models, while MDPs are insufficient to model two strategic agents. 

Compared to MDP synthesis, modeling the human as a strategic agent gives us three benefits. First, it can accurately model strategic humans. Additionally it has the advantages that make reactive synthesis popular \cite{kress2018synthesis}, namely a bounded worst-case and no need for detailed human probability models. The downside is again the greater computational complexity.

\begin{figure*}[t!]
  \centering
  \includegraphics[width=\textwidth]{figs/tic_tac_toe_trace}
  \caption{The game begins with (A) and (B). In state (C) the robot chooses a move that maximizes the probability of human failure under the ``trembling hand'' model. In (D) the human will likely place the object in the bottom center, but has two open neighbor cells. Under the robot policy, the human will have three more chances to fail.}
  \label{fig:tic_tac_toe_trace}
\vspace{0em}
\end{figure*}

\subsection{Scalability}
We test a simple manipulation domain, varying the number of objects and locations. \km{Too much implementation details. Can be removed.} Note that locations 0 and 1 are reserved for the robot and human gripper respectively and the final location indicates termination for that player, so objects can be in locations [2,max-2]. Only one object can be at location 0 or 1 at each time step, otherwise there is no limit on the number of objects at a location.
\km{Very verbose. This can be significantly reduced.}
Prism's default configuration reads in modeling files written in the Prism Modelling Language. This modeling language is designed for structured, heirarchical models, while our models are more naturally represented by a flat structure. Unfortunately the default implementation is quite inefficient on our large flat model files. Prism provides mechanisms for importing MDPs, but not for importing stochastic games, so we implemented this functionality and found that it drastically reduced both runtimes and memory usage. For example, on a scene with 4 objects and 7 locations, runtime decreased from 6000s to 30s and memory usage decreased from approximately 24GB to 1GB. Accordingly, we use our implementation below. Our code has been submitted as a pull request to Prism Games.

We present benchmarks based on the various modeling choices described above. First we compare runtimes of fixed vs probabilistic turn changes \km{The turns are not probabilistic the human termination is} with automata acceptance termination \autoref{table:manip_1_1} and \autoref{table:manip_prob}.

\begin{table}[h]
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
                      & 3 obj 7 loc   & 3 obj 8 loc  & 4 obj 7 loc  &  4 obj 8 loc \\ 
 \hline
 runtime              & 8s            & 36s          &  172s        & 1,343s \\ 
 memory               & 1GB           & 1GB          &  4GB         & 4GB \\ 
 \hline
\end{tabular}
\caption{Runtimes and memory usage on manipulation domain with 1:1 action ratio}
\label{table:manip_1_1}
\vspace{-1em}
\end{table}
It should be noted that with a 1:1 ratio, it is typically not possible for the robot to guarantee task completion. This shortens the runtime.


We experiment with models where the human has a $5\%$ chance of terminating (taking no further actions) at every state. In contrast to \cite{he2019efficient}, where a parameter $k$ was used to constrain the number of human actions, this approach allows greater flexibility and a more intuitive model while still allowing the robot to win the game.

\begin{table}[h]
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
                      & 3 obj 7 loc   & 3 obj 8 loc  & 4 obj 7 loc & 4 obj 8 loc \\ 
 \hline
 runtime              & 11 s          & 59 s         &  208s       & 1,540s       \\ 
 memory               & 1GB           & 1GB          &  4GB        & 4GB     \\ 
 \hline
\end{tabular}
\caption{Runtimes and memory usage on manipulation domain with $5\%$ chance of termination on human actions.}
\label{table:manip_prob}
\end{table}

With 5 blocks and 8 locations, the code takes approximately 15.5hrs to run and uses 32GBs. It should be noted that the majority of Prism's runtime is spent building the reward structure. This illustrates the need for more scalable tools as an important direction for future work.


\subsubsection{Limitations in Our Implementation}
We also examine specifications that affect termination. In previous works and the above tables, termination was determined by reaching the accepting state of an automaton\cite{wells2021probabilistic}. Unfortunately this can give uninuitive results. For example, we may want the robot to clean the room. Under the ``first accepting state'' model of satisfaction, the robot will terminate once the room is clean, even if the human is still present and about to displace an object. Instead we would like the robot to clean the room and remain active until the human leaves. Then the robot should finish cleaning and leave the room. In this case, we can say the robot wins under two scenarios: 

\begin{enumerate}
    \item The human leaves the room and the robot finishes cleaning and then leaves.
    \item The human never leaves the room.
\end{enumerate}

Such a specification can be naturally represented in \ltl. Unfortunately, while Prism Model Checker supports \ltl\ for MDPs, it only provides partial support for \ltl\ on stochastic games. This is not a theoretical limitation, but rather an implementation detail \cite{chen2013automatic}. The authors of Prism are working to fully support \ltl\ on stochastic games. Thus, while stochastic games generalize the earlier models of \cite{he2019efficient, wells2021probabilistic}, our implementation using Prism does not capture the full generality of \ltl\ formulae supported in previous work.

\subsection{Real-world Experiment}
The generality of the stochastic games means a robot using this framework for manipulation can simultaneously solve other problems. For example, consider the classic game of tic-tac-toe where 2 players alternate turns placing markers (in our case yellow \km{Pink!} or \km{and} blue cylinders) in empty cells of a grid. The first player to place three aligned (row, column or diagonal) objects of their color wins \km{No need to explain Tic-Tac-Toe!!}. To make this more interesting, and stochastic, we borrow the concept of the ``trembling hand'' from game theory: a move may accidentally end up in a neighboring cell. Any marker placed is assigned to the closest unoccupied cell.

Using our manipulation framework, we can solve this problem directly \km{directly? What does that mean?}. Code for doing so is available online \cite{wells2021docker}.

% \subsection{Tic-Tac-Toe with ``Trembling Hand''}


% % \ml{should perhaps present this example first with images of an execution since it illustrates the power of stochastic game modeling, and then move to a more general manipulation case study that talks about the computations.}
% The generality of the stochastic games means a robot using this framework for manipulation can simultaneously solve other problems. For example, consider the classic game of tic-tac-toe where 2 players alternate turns placing markers (in our case yellow or blue cylinders) in empty cells of a grid. The first player to place three aligned (row, column or diagonal) objects of their color wins.

% Tic-tac-toe can be easily solved using min-max, but the robot may fail to physically make the move requested by the min-max solver. Suppose the robot places objects only approximately, and objects are always ``assigned'' to the closest available cell. Then if we know the probability of object placements (say a normal distribution with standard deviation of 1-cell width), we can use a stochastic game to model optimal robot play.

% This differs from reactive synthesis, where the robot and human would assume perfect play from their opponents. Then each would move in the first available non-losing cell according to some lexicographic order (say top left to bottom right). By contrast, using our model of stochastic games allows us model possible human failures. Then the robot can move so as to maximize the chances of human failure. While the robot may not be able to distinguish between human actions that are intended to move in one cell but moved somewhere else and strategic mistakes, the robot can use some probability of ``non-optimal human play'' (say a 1\% chance that the human will move to an open cell uniformly at random each turn).

% \begin{table}[h]
% \begin{tabular}{ |c|c|c| } 
%  \hline
%                       & PMax Robot Win   & PMin Human Win   \\ 
%  \hline
%  runtime              & $1.3$ s          & $1.3$ s             \\ 
%  memory               & 1GB           & 1GB              \\ 
%  \hline
% \end{tabular}
% \caption{Runtimes and memory usage for tic-tac-toe with two specifications. On the left, a tie is considered a failure, while on the right a tie is considered a success.}
% \label{table:tic_tac_toe}
% \end{table}

% Here we see that stochastic games offer a different framework than min-max search. The robot can be told to either maximize its chance of winning or to minimize the human's chance of winning (see \autoref{table:tic_tac_toe}). Perhaps counter-intuitively, these strategies differ. Even more interesting behavior could result from modeling probabilities of different human errors, where the robot could play a move that would be sub-optimal against a perfect opponent, but is optimal with respect to probable human errors.




==> sections/old_modeling.tex <==
\section{Modeling}
\label{sec:modeling}



\begin{table}
\begin{center}
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
 Stochastic Game        & Robotics Domain        \\
 \hline
 Discrete states + actions        & Continuous states + actions      \\
 Turn-based             & Free-form actions      \\
 Limited human model & Flexible human capabilities \\
 Specified termination  & Unconstrained termination     \\
 \hline
\end{tabular}
\caption{Primary challenges to modeling human-robot manipulation as a 2-player stochastic game.}
\label{table:modeling_challenges}
\end{center}
\end{table}


\begin{figure}[h]
    \centering
    \begin{subfigure}{0.3\columnwidth}
        \includegraphics[width=\textwidth]{figs/abs_init_state}%
        % \caption{}
        \label{fig:start_state}
    \end{subfigure}
    \qquad \quad
    \begin{subfigure}{0.3\columnwidth}
        \includegraphics[width=\textwidth]{figs/abstract_robot_state}
        % \caption{}
        \label{fig:robot_act}
    \end{subfigure}
        \qquad \quad
    \begin{subfigure}{0.3\columnwidth}
        \includegraphics[width=\textwidth]{figs/abstract_human_state}
        % \caption{}
        \label{fig:human_act}
    \end{subfigure}
    \caption{Manipulation domain: (left) the initial state. (right) the result of a robot ``pick'' action. (center) the result of an attempted robot ``place'' action that was interrupted by the human.}
    \label{fig:abs_manip}
\end{figure}


% In this paper we deal with two-player, turn-based stochastic games (for brevity referred to simply as \emph{stochastic games}). Tools such as Prism Games \cite{kwiatkowska2020prism} can handle more players, (using the coalition operator to define two teams) as well as concurrent rather than turn-based games. We use turn-based, two-player games because two-players suffices for modeling our scenarios and concurrent games are more computationally complex to solve.

In section \autoref{sec:preliminaries}, we discussed how previous works \cite{He:IROS:2017, He:RAL:2018, he2019efficient, wells2021probabilistic} approached human-robot manipulation. We listed the main challenges to modeling human-robot manipulation in these methods in \autoref{table:modeling_challenges}. Prior models assumed the human is either adversarial or stochastic, but could not be mixed to accurately match the needs of our problem. Here we discuss how strategic and stochastic elements of the human and robot are combined to form a two-player stochastic game.

We follow prior approaches to map continuous states and actions to discrete states and actions. For stochastic games, we still need new approaches to address most of the challenges from \autoref{table:modeling_challenges}:

\begin{enumerate}
    \item Transform free-form actions into a turn-based game
    \item Weaken assumptions on human behavior
    \item Specify termination in human-robot manipulation
\end{enumerate}

We present our approaches to these challenges for stochastic games below:

% \subsection{2.5-player game}
% In our model, we have two strategic agents as well as stochastic effects caused by ``nature.'' The stochastic effects can apply to both, one or neither player. When stochastic effects apply to at least one player, we have a 2.5-player game (one system player, one environment player and the half-player of ``nature'').

% For the strategic players, we follow the models of prior works \cite{he2019efficient}. The robotic agent follows a standard pick-place domain, which typically can be encoded in 
% PDDL. The human player has the same abilities, but is assumed to move relatively quickly compared to the robot. Additionally, as a modeling assumption, we do not allow the human to hold onto an object (as in prior works \cite{he2019efficient}). Thus we model the robot's gripper but no human gripper.

\subsection{Modelling Manipulation as a Turn-Based Game}
\label{sec:allocating_turns}
In free-form human-robot interaction, there is no notion of a ``turn.'' Tools such as Prism Games \cite{kwiatkowska2020prism} can handle concurrent rather than turn-based games, but with greater computational cost. Because scalability is already a significant challenge, we stick to turn-based games.

We essentially need to answer two questions: Whose turn is it? And what can an agent do in this (one) turn?

In prior works, the human is typically assumed to move faster than the robot, leading to multiple human moves per robot move. We follow this assumption and examine several models of turn allocation. To maximize human flexibility, we always allow the human to act. Because we do not want the robot to waste time, the robot always attempts to act. As in \cite{He:IROS:2017}, we assume certain robot actions are ``atomic'' while giving the human actions priority over all non-atomic actions. Here, as in previous work, the atomic robot actions are grasp and place (not including the transit or transfer preceding the opening / closing of the gripper). We try to grant the human greater flexibility than the robot in our models. E.g., by allowing multiple human actions in quick succession or by giving the human priority over the robot \autoref{fig:toy_example}.

At each state, the robot consults its policy to find the optimal action, then attempts to perform that action. If the state updates before the robot completes its action, it considers the human turn finished and again consults its policy to find the optimal action in the new state. If the human acts again, the robot proceeds in the same way. The human has exceeded its action limits (see below), but so long as the resulting state is included in the robot policy, the robot will still have an optimal response (under the modeling assumptions) for the new state.


Once we have chosen a way to model actions, and under our assumptions about discrete states and atomic action executions, we can create a turn-based stochastic game.

A partial 2.5-player stochastic game for our manipulation domain is shown in \autoref{fig:stochastic_game}.

\begin{figure}[h!]
    \label{ex:example_stochastic_game}
        \centering
        \begin{tikzpicture}[auto,node distance=3cm,on grid,line width=0.4mm]
        %   \tikzstyle{round}=[thick,draw=black,circle]
          
    
            \node[circle,draw,state,inner sep=1pt,minimum size=0pt] (s0) {\includegraphics[width=13mm]{figs/arch_init}};
            \node[rectangle,draw,inner sep=4pt,minimum size=0pt] (s1) [below left=of s0] {\includegraphics[width=13mm]{figs/arch_grasped}};
            \node[rectangle,draw,inner sep=4pt,minimum size=0pt] (s2) [below right= of s0] {\includegraphics[width=13mm]{figs/arch_other}};
            \node[circle,draw,state,accepting,inner sep=1pt,minimum size=0pt] (s3) [below =2.1cm of s1] {\includegraphics[width=13mm]{figs/arch_final}};
            \node[circle,draw,state,inner sep=1pt,minimum size=0pt] (s4) [below left=of s2] {\includegraphics[width=13mm]{figs/arch_other}};
            \node[circle,draw,state,inner sep=1pt,minimum size=0pt] (s5) [below right=of s2] {\includegraphics[width=13mm]{figs/arch_another}};
    
            \path[->]       (s0) edge (s1)
                            (s0) edge (s2);
            \path[->]       (s1) edge (s3);
            \path[->]       (s2) edge (s4)
                            (s2) edge (s5);
    
            % \path[->] 	(s0) edge [bend left=55] node [above] {\footnotesize 0.9} (s1)
            %             (s0) edge [bend left=55] node [below] {\footnotesize \emph{grasp blue}} (s1)
            %             (s0) edge [in=75,out=55,loop,pos=0.7] node [left=1mm] {\footnotesize 0.1} ()
            %             (s0) edge [bend right=50] node [left=1mm] {\footnotesize 0.9} (s2)
            %             (s0) edge [bend right=50] node [right=0.5mm] {\footnotesize \emph{grasp yellow}} (s2)
            %             (s0) edge [in=210,out=220,loop,pos=0.9] node [left=1mm] {\footnotesize 0.1} ();
            % \path[->] 	(s1) edge node [above,pos=0.7] {\footnotesize 0.9} (s0)
            %             (s1) edge node [below] {\footnotesize \emph{put blue}} (s0)
            %             (s1) edge [in=165,out=180,loop,pos=0.9] node [above=1mm] {\footnotesize 0.1} ()
            %             (s1) edge node [above,pos=0.7] {\footnotesize 0.9} (s3)
            %             (s1) edge node [below,pos=0.5] {\footnotesize \emph{stack blue}} (s3)
            %             (s1) edge [in=15,out=0,loop,pos=0.9] node [above=1mm] {\footnotesize 0.1} ();
            % \path[->] 	(s2) edge [bend right=45,pos=0.7] node [right=1mm] {\footnotesize 0.9} (s0)
            %             (s2) edge [bend right=45,pos=0.4] node [right=1mm] {\footnotesize \emph{put yellow}} (s0)
            %             (s2) edge [in=30,out=45,loop,pos=0.9] node [right=0.25mm] {\footnotesize 0.1} ();
    
            %% loop for the action
            % \path pic[draw, angle radius=7mm,"\vphantom{g} \footnotesize{$a_1$}",angle eccentricity=1.3] {angle = s2--s0--s1};
            
        \end{tikzpicture}
        \caption{Partial stochastic game for pick-and-place domain. Transitions can have probabilities to model stochastic effects, errors or random choices.}
        \label{fig:stochastic_game}
    \vspace{0em}
\end{figure}

The actions taken in circular states are controlled by the system and those taken in rectangular states are controlled by the environment. The same action could stochastically lead to different possible states (e.g., in the above the robot's first action could attempt to pickup a cylinder from the initial state and stochastically determine whether to grasp the yellow or the blue cylinder).



% \subsection{Synchronization}
% We need to synchronize so that the human and robot agree on whose turn it is.  We do this by adding a ``lock'' variable that indicates whose turn it is. Depending on our modeling choices from \autoref{sec:alloc_turns}, this can either be handed off after a bounded number of moves or probabilistically.
% We compare two models. In one, the human and robot alternate turns. In the other the human can take an arbitrary number of consecutive turns.

% Test human veto vs probability of robot failure.

\subsection{Weakening Assumptions (Limits) on Human Behavior}

Previous works \cite{He:IROS:2017, He:RAL:2018, he2019efficient} had to include additional restrictions such as limiting the number of actions or the rate of actions. A limit \emph{k} is placed on the total number of human actions to ensure the specification is realizable. This limit is unintuitive and somewhat unrealistic. For example, suppose the model assumes the human  makes at most 30 actions ($k = 30$). Then during execution, once the robot observes the $30^{th}$ action, it will act as though the human will no longer interfere. Unfortunately, unless there is some external reason for this limit, the robot should arguably assume the human is \emph{more} likely to interfere because it has observed this happen $30$ times already.

We generalize this as a \emph{ratio} of human and robot actions. For example we could allow 1 human action for every 2 robot actions (denoted by $2:1$). We implement this using counters that reset every time the game changes control from one player to another. So a player cannot ``skip'' turns now in order to take more consecutive turns later. This means, $4:2$ is not necessarily the same as $2:1$.

We also present a model using a probability of handing control from one player to another. This implies a probabilistic limit, but avoids setting a hard limit on action for either player. For example, instead of limiting the human to $k=30$ actions, we could give the human a probability of stopping after each action $p_k = 1/30$. In our experiments, we find this more flexible model leads to only minor extra computational cost.

\subsection{Termination}
Finally, we have to define some notion of who wins the game. In previous works, this was done by accepting finite prefixes. This can be uninuitive, for example a robot asked to clean the room will stop once the room is cleaned, even if the human is approaching some object to displace it. In our new model, we would like to allow the human and robot to ``negotiate'' termination so that the robot only considers the task complete when the human agrees.

For a given \ltlf\ specification (e.g., eventually construct some object), synthesis reduces to solving a stochastic game for a reachability objective that corresponds to reaching the accepting state of the deterministic finite automata expressed by the \ltlf\ specification. 

Our \ltlf specifications can be made into reachability objectives. Then there exists an optimal memoryless, deterministic policy for each player. The game can be solved using value iteration until some convergence criteria is met \cite{chen2013automatic}. How many iterations this will take is an open question, and solving stochastic games with reachability objectives lies in the complexity class $NP \cap coNP$ \cite{condon1993algorithms}.

==> sections/old_preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

We begin by discussing our model of robotic manipulation domain. Then we discuss logical specifications for these domains and stochastic models used to reason over logical specifications. We follow the frameworks used in \cite{He:IROS:2017, He:RAL:2018, he2019efficient, wells2021probabilistic} for solving human-robot manipulation problems using reactive or probabilistic synthesis. We briefly overview these approaches since our work builds on them. Then we define stochastic games, but save discussion of specific techniques for modeling manipulation as a stochastic games for the next section.

\subsection{Manipulation Domain}

As a starting point, we use a manipulation domain abstraction based off of \cite{He:RAL:2018}. 


\begin{definition}[Abstraction of a Manipulation Domain]
    \label{def:manip_domain_abstraction}
	An \emph{abstract manipulation domain} is a tuple: $G_{det}=(S, s_0, A_s, A_e, T, AP, L)$ where,
	\begin{itemize}
		\item $S$ is a finite set of states,
		\item $s_0 \in S$ is the initial state,
		\item $A_s$ is the finite set of system (robot) actions,
		\item $A_e$ is the finite set of environment (human) actions,
		\item $T : S \times (A_s \cup A_e) \mapsto S$ is the transition function,
		\item $AP$ is the set of task-related atomic propositions,
		\item $L : S \mapsto 2^{AP}$ is the labeling function that maps each state to a set of atomic propositions.
	\end{itemize}
\end{definition}

As an example, consider the abstract manipulation domain depicted in \autoref{fig:toy_example}. There are two agents, a robot and a human. Each agent can change the state of the world, albeit under some restrictions. For the robot, these restrictions follow typical PDDL pick-place domains \cite{pddl}. For example, the robot cannot pickup an object while it is supporting another object \autoref{fig:toy_example}. For the human, various assumptions are introduced to make the problem tractable \cite{he2019efficient, wells2021probabilistic}. We discuss how stochastic games allow us to relax these assumptions in \autoref{sec:modeling}.


% \begin{figure}[h]
%   \begin{center}
%     \includegraphics[width=0.3\textwidth]{figs/abs_init_state}
%   \end{center}
%   \caption{Abstract initial state}
%   \label{fig:start_state}
% \end{figure}

% \begin{figure}[h]
% 	\begin{center}
% 	  \includegraphics[width=0.3\textwidth]{figs/abstract_robot_state}
% 	\end{center}
% 	\caption{Abstract state after robot action}
% 	\label{fig:robot_act}
% \end{figure}

% \begin{figure}[h]
% 	\begin{center}
% 	  \includegraphics[width=0.3\textwidth]{figs/abstract_human_state}
% 	\end{center}
% 	\caption{Abstract state after robot tries to place the yellow object and the human interrupts}
% 	\label{fig:human_act}
% \end{figure}


Once we have a model of a manipulation domain, we next need some formal way to express properties of ``runs'' (executions) through this domain.
% As in \cite{wells2021probabilistic}, we use ``missing'' objects to denote objects in the ``Else'' region (see \autoref{fig:toy_example}).

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.25\columnwidth}
        \includegraphics[width=\textwidth]{figs/arch_locs}%
        % \caption{}
        \label{fig:toy_example_setup}
    \end{subfigure}
    \qquad \quad
    \begin{subfigure}{0.25\columnwidth}
        \includegraphics[width=\textwidth]{figs/arch_init}
        % \caption{}
        \label{fig:toy_example_initial}
    \end{subfigure}
    \vspace{-1em}
    \caption{Manipulation domain: (left) the locations of interest, where the Else location ($Loc_1$) contains all objects not otherwise shown.
    (right) Initial state with red and yellow blocks at $Loc_2$ and $Loc_3$ and the blue block at $Loc_1$.}
    \label{fig:toy_example}
\end{figure}

\subsection{Linear Temporal Logic over Finite Traces}
Linear temporal logic (\ltl) \cite{pnueli1977temporal} is a popular formalism used to specify temporal properties over infinite horizons. In robotics, we are frequent interested in \ltl interpreted over finite traces (\ltlf) \cite{de2013linear}. 

\begin{definition}[\ltlf Syntax]
	An \ltlf formula is built from a set of atomic propositions $AP$ and is closed under the Boolean connectives as well as the ``next'' operator $X$ and the ``until'' operator $U$:
	\[
		\ltlfphi ::= \top   \mid   p   \mid   (\neg \ltlfphi)   \mid   (\ltlfphi_1 \wedge \ltlfphi_2)   \mid   (X \ltlfphi)  \mid  (\ltlfphi_1 U \ltlfphi_2)
	\]
	where $p \in AP$, $\top$ is ``true'' or a tautology, and $\neg$ and $\wedge$ are the ``negation'' and ``and'' operators in Boolean logic respectively.
\end{definition}

\noindent
The common temporal operators ``eventually'' ($F$) and ``globally'' ($G$) are defined as: $F \, \ltlfphi = \top \, U \, \ltlfphi$ and $G \, \ltlfphi = \neg F\, \neg \ltlfphi$.

We can use \ltlf to express a property such as ``this construction task must be completed safely.''

\begin{example}[Example \ltlf specification]

Consider the \ltlf formula

$ F\ constructed \wedge G\ \neg\ safety\_violation $

Read ``Eventually $Constructed$ and Globally not $safety\_violation$''. This could be used to specify that the robot must finish construction in finite time and while doing so must not move to an unsafe state (a state where the robot is too close to the human).

\end{example}

For a more thorough treatment of \ltlf, see \cite{de2013linear, de2015synthesis} or similar.

% The semantics of \ltlf are defined as follows.

% \begin{definition}[\ltlf Semantics]
% 	The semantics of an \ltlf \hspace{0.5mm}formula are defined over finite traces. A trace $\rho$ is a word in $(2^{AP})^*$. Let $|\rho|$ denote the length of trace $\rho$ and $\rho[i]$ be the $i^{th}$ symbol of $\rho$. Further, $\rho, i \models \ltlfphi$ is read as: ``the $i^{th}$ step of trace $\rho$ is a model of $\ltlfphi$.'':
% 	\begin{itemize}
% 		\item $\rho , i \models \top;$
% 		\item $\rho , i \models p$ iff $p \in \rho[i];$
% 		\item $\rho , i \models \neg \ltlfphi$ iff $\rho, i \not \models \ltlfphi;$
% 		\item $\rho , i \models \ltlfphi_1 \wedge \ltlfphi_2$, iff, $\rho, i \models \ltlfphi_1$ and $\rho, i \models \ltlfphi_2;$
% 		\item $\rho , i \models X \ltlfphi$ iff $|\rho| > i+1$ and $\rho, i+1 \models \ltlfphi;$
% 		\item $\rho , i \models \ltlfphi_1 U \ltlfphi_2$ iff $\exists j$ s.t. $ i \leq j < |\rho|$ and $\rho, j \models \ltlfphi_2$ and $\forall k$, $i \leq k < j$, \; $\rho, k \models \ltlfphi_1$,
% 	\end{itemize}
% \end{definition}
% Finite trace $\rho$ satisfies $\ltlfphi$, denoted by $\rho \models \ltlfphi$, if $\rho, 0 \models \ltlfphi$.
% An $LTL_f$ formula $\ltlfphi$ defines a language $\mathcal{L}(\ltlfphi)$ over the alphabet $2^{AP}$. $\mathcal{L}(\ltlfphi)$ is a regular language, more specifically, $\mathcal{L(\ltlfphi)} = \{\rho \in (2^{AP})^* \mid \rho \models \ltlfphi\}$. 
% % (recall that \ltlf has the expressivity of star-free regular languages).



% \subsection{Probabilistic Abstraction of Manipulation Domain}
% We extend our manipulation domain abstraction $G_{prob}$ by introducing non-deterministic actions to be controlled by the environment.

% \begin{definition}[Probabilistic Abstraction of a Manipulation Domain]
% The probabilistic abstraction of a manipulation domain is a tuple: $G_{stoch\_game}=(S, s_0, A_s, A_e, T_e, AP, L, P_s, P_e)$ where $S, s_0, A_s, A_e, AP$ and $L$ are defined as in  \autoref{def:manip_domain_abstraction} and
% \begin{itemize}
% 	\item $S$ is a finite set of states,
% 	\item $s_0 \in S$ is the initial state,
% 	\item $A_s$ is the finite set of system (robot) actions,
% 	\item $A_e$ is the finite set of environment (human) actions,
% % 	\item $T : S \times (A_s \cup A_e) \mapsto S$ is the transition function,
% 	\item $T_e$ gives the result of applying human action $act_e \in A_e$ at state $s \in S$. $T_e: S \times A_e \times S \to \{0,1\}$.
% 	\item $AP$ is the set of task-related atomic propositions,
% 	\item $L : S \mapsto 2^{AP}$ is the labeling function that maps each state to a set of atomic propositions.
% 	\item $P_s$  is a probability function $P_s: S \times A_s \times S \to [0,1]$ that gives the probability distribution of effects of system (robot) actions as the probability $P_s(s_{i+1} \mid act_s, s_i)$,
% 	\item $P_e$ is a probability function $P_e: S \times A_e \to [0,1]$ that gives the probability of an environment (human) action being applied at the current state $P_e(act_e \in A_e \mid s_i)$.
% \end{itemize}
% \end{definition}

% Description.
\subsection{Reactive Models}
In \cite{He:IROS:2017, He:RAL:2018, he2019efficient}, reactive synthesis is used to construct worst-case optimal behavior for the robot by assuming adversarial human actions. This works well in scenarios where high-assurance is needed (e.g., there is a possibility of harming a human, so we need to guarantee safety) and where stochastic effects are absent or can be ignored (e.g., the robot performs actions with high accuracy, so outcomes are deterministic or nearly so). Because reactive synthesis considers the worst case, fairly strong and arguably unnatural assumptions are made about human behavior. For example, in \cite{He:IROS:2017, He:RAL:2018, he2019efficient}, the human is limited to a fixed number of actions $k$ to ensure specifications are realizable. Using stochastic games, we can remove this and other assumptions.


\begin{example}
For a purely strategic human, the manipulation domain becomes a deterministic transition system.

\begin{figure}[h]
    \vspace{0em}
        \centering
        \scalebox{0.94}{
        \begin{tikzpicture}[auto,node distance=2.5cm,on grid,line width=0.4mm]
            \tikzstyle{round}=[thick,draw=black,circle]
    
            % \node[state, label={\footnotesize $\emptyset$}] (s0) {$\langle 1,2,3 \rangle$};
            \node[state,inner sep=1pt,minimum size=0pt] (s0) {\includegraphics[width=11mm]{figs/arch_init}};
            \node[state,inner sep=1pt,minimum size=0pt] (s1) [right=of s0] {\includegraphics[width=11mm]{figs/arch_grasped}};
            \node[state,inner sep=1pt,minimum size=0pt] (s2) [below=1cm of $(s0)!0.5!(s1)$] {\includegraphics[width=11mm]{figs/arch_other}};
            \node[state,accepting,inner sep=1pt,minimum size=0pt] (s3) [right=of s1] {\includegraphics[width=11mm]{figs/arch_final}};		
    
            \path[->] 	(s0) edge node {} (s1)
                        (s0) edge node {} (s2);
            \path[->] 	(s1) edge [bend right=45] node [above] {} (s0)
                        (s1) edge node [above] {} (s3);
            \path[->] 	(s2) edge [bend left=45] node [below] {} (s0);
                        
        \end{tikzpicture}
        }
        \caption{Example portion of abstraction of manipulation domain for a deterministic pick-and-place domain. 
        % The state-space is explained in \autoref{fig:toy_example}.
        }
        \label{fig:example_deterministic}
\end{figure}
\end{example}

\subsection{Stochastic Models}
In reactive synthesis, human-robot interaction was modeled as a game with two strategic players \cite{he2019efficient}. This works well for scenarios with little or no stochasticity or where stringent guarantees are required; however, the 2-player model was limiting in several ways. First it requires us to reason about the worst-case human behavior. Second in order to win the game, we need to impose some limit, e.g., $k$ human actions. Finally, it cannot express stochastic behavior, such as actions where we have observed a statistical failure rate.

To address these limitations, \cite{wells2021probabilistic} proposed modeling human-robot manipulation using MDPs, which are 1.5-player games. This is useful for expressing stochastic interactions, but cannot express two strategic agents.

\subsubsection{Markov Decision Process}

To build \mdpmanip from $G_{det}$, a combined probability distribution was built from the probabilities of human actions and of the effects of robot actions. Under this model, the human is not strategic, so each node in the MDP will have only one human action. An example of a simplified MDP with only the human actions is shown in \autoref{fig:examplemdp}. Note that the human cannot alter the robot's end-effector:
\begin{example}
\begin{figure}[h]
    \vspace{-1em}
    \label{ex:example_mdp_human}
        \centering
        \begin{tikzpicture}[auto,node distance=3cm,on grid,line width=0.4mm]
          \tikzstyle{round}=[thick,draw=black,circle]
    
            \node[state,inner sep=1pt,minimum size=0pt] (s0) {\includegraphics[width=13mm]{figs/arch_init}};
            \node[state,accepting,inner sep=1pt,minimum size=0pt] (s1) [right=3.5cm of s0] {\includegraphics[width=13mm]{figs/arch_final}};
            \node[state,inner sep=1pt,minimum size=0pt] (s2) [below=2.1cm of s0] {\includegraphics[width=13mm]{figs/arch_red_empty}};
            \node[state,inner sep=1pt,minimum size=0pt] (s3) [below=2.1cm of s1] {\includegraphics[width=13mm]{figs/arch_empty_yellow}};		

            \node[state,inner sep=1pt,minimum size=0pt] (s4) [above=2.1cm of s0] {\includegraphics[width=13mm]{figs/arch_another}};
            \node[state,inner sep=1pt,minimum size=0pt] (s5) [above=2.1cm of s1] {\includegraphics[width=13mm]{figs/arch_yellow_red}};
            \node[draw=none,fill=none, right=1.5cm of s4] {\Large\dots};
    
            \path[->] 	(s0) edge [in=180,out=0,pos=0.8] node [above] {\footnotesize 0.15} (s1)
                        (s0) edge [in=55,out=0,pos=0.8] node [left=1mm] {\footnotesize 0.15} (s2)
                        (s0) edge [in=125,out=0,pos=0.8] node [left=1mm] {\footnotesize 0.15} (s3)
                        (s0) edge [in=12,out=2,loop,pos=0.9] node [above=1mm] {\footnotesize 0.4} ()
                        (s0) edge [in=340,out=0,pos=1] node [above=0.25mm, right=1mm] {\footnotesize 0.03} (s4)
                        (s0) edge [in=195,out=0,pos=0.9] node [below=1mm] {\footnotesize 0.03} (s5);
            % \path[->] 	(s1) edge node [above] {\footnotesize 0.9} (s0)
            %             (s1) edge [in=195,out=180,loop,pos=0.9] node [below=1mm] {\footnotesize 0.1} ()
            %             (s1) edge node [above,pos=0.7] {\footnotesize 0.9} (s3)
            %             (s1) edge [in=15,out=0,loop,pos=0.9] node [above=1mm] {\footnotesize 0.1} ();
            % \path[->] 	(s2) edge [bend right=30,pos=0.9] node [right=1mm] {\footnotesize 0.9} (s0)
            %             (s2) edge [in=110,out=100,loop,pos=0.9] node [left=0.25mm] {\footnotesize 0.1} ();
            %% loop for the action
            % \path pic[draw, angle radius=7mm,"\vphantom{g} \footnotesize{$a_1$}",angle eccentricity=1.3] {angle = s2--s0--s1};
            
        \end{tikzpicture}
        \caption{Example portion of an MDP encoding human actions. In the top row, the human has moved two blocks. In the remaining states, the human has moved one or no blocks.}
        \label{fig:examplemdp}
    \vspace{-1em}
\end{figure}
The human has probabilities for moving none, one or several of the blocks in \autoref{fig:examplemdp}. The robot can concurrently attempt to move blocks, deferring to the human in the case of conflict. The result is an MDP with many possible transitions between states, where each transition can encode several block motions. For example in the top left, the robot may have tried to grasp the blue block, and have been overridden by the human. The human moved the yellow and then the blue block in one transition.
\end{example}

We would like to combine the expressivity of both models by considering two strategic players \em the human and the robot \em both with stochastic actions.

\subsubsection{Stochastic Games}
Here, we formally define stochastic games, which we will use to model human-robot manipulation in \autoref{sec:modeling}.
\begin{definition}[Stochastic Game]
A stochastic game is a tuple $G = (S, s_0, A, T, C, AP, L)$ where $S, s_0, AP$ and $L$ are as in \autoref{def:manip_domain_abstraction} and :
\begin{itemize}
    \item $A$ is the finite set of actions
    \item $T: S \times A \times S \mapsto [0,1]$ is the probabilistic transition relation
    \item $C: S \mapsto \mathbb{N}$ designates which player controls the choice of action at each state
\end{itemize}
We say $G$ is a two-player stochastic game when $C : S \mapsto \{0,1\}$.
\end{definition}
Intuitively, a stochastic game is similar to an MDP except that there are two (or more) independent strategic agents that take turns making choices. For more details on stochastic games, see \cite{kwiatkowska2020prism, fundberg1991game}

\begin{definition}[Path through a Stochastic Game]
A path through a stochastic game is a finite sequence of states
$\lambda : s_0, ..., s_n$
\end{definition}

\begin{definition}[Policy for a Stochastic Game]
A policy for a stochastic game is a function from a history of states and an action to a probability.
$\sigma : \lambda \times A \mapsto [0,1]$
such that for any $\lambda$, $\sum_A \sigma(\lambda act) = 1$
\end{definition}

For two player stochastic games with a reachability objective memoryless, deterministic strategies suffice \cite{chen2013automatic}. 

\subsection{Modeling Challenges}

Considering \autoref{table:modeling_challenges}, prior works in reactive or probablistic synthesis for robot manipulation solve the first challenge, by giving a means of mapping discrete states and actions into continuous states and actions \cite{He:RAL:2018, he2019efficient, wells2021probabilistic}. In brief, we model the continuous world by grouping locations into ``regions of interest.'' These include a ``end-effector'' region representing the robot's gripper and an ``else'' region representing all locations not particularly specified. Robot actions are divided into ``atomic'' and ``non-atomic'' actions, where atomic actions are considered discrete and uninterruptable while non-atomic actions can be interrupted by the human. For more details, see \cite{He:RAL:2018}, which gives a method for automated construction of such an abstraction.

We can apply this method to modeling human-robot manipulation as a stochastic game. The remaining challenges from \autoref{table:modeling_challenges} are: moving from free-form to turn-based interactions, providing a limited model of inherently flexible human capabilities and specifying termination in our model either pose new challenges for stochastic games or can benefit from the more flexible modeling capabilities of stochastic games. We address these challenges in \autoref{sec:modeling}.


==> sections/old_results.tex <==
\section{Results}
Stochastic games subsume the expressivity of both reactive and probabilistic synthesis. Unfortunately, they bring a new level of challenges in scalability. We present simple benchmarks based on experiments from \cite{wells2021probabilistic}.

We run our test using the Prism Model Checker \cite{kwiatowska2011prism}, an open-source tool implemented in Java. We make small modifications to remove a performance bottleneck when importing models and these changes have been submitted as a pull request to Prism. All experiments are run on a Ryzen 9 5950x and RAM limits are set for the JVM via command line arguments (see below). Our experiments are available online \cite{wells2021github}. We have also created Docker images to aid reproducibility \cite{wells2021docker}.

We test a simple manipulation domain, varying the number of objects and locations. Note that locations 0 and 1 are reserved for the robot and human gripper respectively and the final location indicates termination for that player, so objects can be in locations [2,max-2]. Only one object can be at location 0 or 1 at each timestep, otherwise there is no limit on the number of objects at a location.

We present benchmarks based on the various modeling choices described above. For reference, see table 

% \begin{center}
% \begin{tabular}{ |c|c|c| } 
%  \hline
%  scene      & 3 obj 7 loc  & 3 obj 8 loc  & 4 obj 7 loc & 4 obj 8 loc\\ 
%  \hline
%  num states & 9,200        & 21,960       & 48,000      & --         \\ 
%  num transitions & 45,840  & 129,210      & 48,000      & --         \\ 
%  runtime    & 520s         & 1464s        & 6063s       & --         \\ 
%  memory     & 2GB          & 4GB          & 8GB         & OOM        \\
%  \hline
% \end{tabular}
% \end{center}


% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%  scene      & 3 obj 7 loc  & 3 obj 8 loc  & 4 obj 7 loc & 4 obj 8 loc\\ 
%  \hline
%  num states & 9,200        & 21,960       & 48,000      & --         \\ 
%  num transitions & 45,840  & 129,210      & 48,000      & --         \\ 
%  runtime    & 520s         & 1464s        & 6063s       & --         \\ 
%  memory     & 2GB          & 4GB          & 8GB         & OOM        \\
%  \hline
% \end{tabular}
% \end{center}

% This is with the explicit engine. With the symbolic engine, 4 objects and 7 locations take 6250s.

% We also consider models with a probability of human termination:

% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%  scene      & 3 obj 7 loc  & 3 obj 8 loc  & 4 obj 7 loc & 4 obj 8 loc\\ 
%  \hline
%  num states & 9,200        & 21,960       & 48,000      & --         \\ 
%  runtime    & 285s         & 2020s        & 6871s       & --         \\ 
%  memory     & 2GB          & 8GB          & 28GB         & OOM        \\
%  \hline
% \end{tabular}
% \end{center}

% We also consider a model where the human does not have to end it's turn (this is equivalent to allowing one transition with more effects but still requiring a handoff of the turn).

% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%  scene      & 3 obj 7 loc  & 3 obj 8 loc  & 4 obj 7 loc & 4 obj 8 loc\\ 
%  \hline
%  num states & 9,200        & 21,960       & 48,000      & --         \\ 
%  runtime    & 250s         & 1510s        & ?s       & --         \\ 
%  memory     & 2GB          & 10GB          & ?GB         & OOM        \\
%  \hline
% \end{tabular}
% \end{center}

We also examine specifications that affect termination. For example, we may want the robot to clean the room and remain active until the human leaves. Then the robot should finish cleaning and leave the room. In this case, we can say the robot wins under two scenarios: 

\begin{enumerate}
    \item The human leaves the room and the robot finishes cleaning and then leaves.
    \item The human never leaves the room.
\end{enumerate}

In contrast to \cite{he2019efficient}, where a parameter $k$ was used to constrain the number of human actions, this approach allows greater flexibility and a more intuitive model while still allowing the robot to win the game.

% \subsection{Gridworld}

% We consider a gridworld domain with one robot and one human, each moving in the cardinal directions.

% % \begin{center}
% % \begin{tabular}{ |c|c|c|c|c| } 
% %  \hline
% %  scene      & 10x10      & 25x25   & 50x50     & ?\\ 
% %  \hline
% %  num states & 1,105      & 60,000  & ?    & --         \\ 
% %  runtime    & 5s         & 1552s   & ?s     & --         \\ 
% %  memory     & 1GB        & 4GB     & ?GB      & OOM        \\
% %  \hline
% % \end{tabular}
% % \end{center}

% 99\% of runtime is spent in model construction.

% Even a deterministic model for the robot with a deterministic human model with one action per state takes roughly this long. 1552s for model construction on a 25x25 game (60,000 states, 145200 transitions=choices).

% For an MDP (identical to the deterministic model), the construction takes about 38s on a 25x25 game. (30,000 states, 253,910 transitions=choices).


% Maybe due to search through game states having too many duplicates.
% Total added states: 9199
% Total viewed states: 169619


% Importing games is much faster.


\begin{center}
\begin{tabular}{ |c|c|c| } 
 \hline
 scenario                 & old runtime    & new runtime \\ 
 \hline
 gridworld                & 30s            & 0.5s   \\ 
 cleaning room prob term  & 6000s          & 30s  \\ 
 cleaning room alt turns  & 5600s          & 5s   \\
 \hline
\end{tabular}
\end{center}


==> sections/preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.3\columnwidth}
        \includegraphics[width=\textwidth]{figs/abs_init_state}%
        % \caption{}
        \label{fig:start_state}
    \end{subfigure}
    \qquad \quad
    \begin{subfigure}{0.3\columnwidth}
        \includegraphics[width=\textwidth]{figs/abstract_robot_state}
        % \caption{}
        \label{fig:robot_act}
    \end{subfigure}
        \qquad \quad
    \begin{subfigure}{0.3\columnwidth}
        \includegraphics[width=\textwidth]{figs/abstract_human_state}
        % \caption{}
        \label{fig:human_act}
    \end{subfigure}
    \caption{Manipulation domain: (left) the initial state. (right) the result of a robot ``pick'' action. (center) the result of an attempted robot ``place'' action that was interrupted by the human.}
    \label{fig:abs_manip}
\end{figure}

 We begin by discussing our model of robot manipulation. Then we discuss logical specifications for these domains and stochastic models used to reason over logical specifications.

 \ml{make this the problem formulation section.  First introduce robot manipulation domain as an MDP, uncertain actions, e.g., dropping objects, failing to grasp, ctc.  Then, Say we assume there is a human present in the environment... we only consider human actions as moves of the objects... and some more information... we also known that human makes decisions according to a latent objective and some data exists from past scenarios... Define robot's task as LTLf formula....  define the problem as: synthesize a strategy for the robot to achieve its task.   \\
 Approach: abstract to stochastic games. 
 }

\subsection{Manipulation Domain}

As a starting point, we use a manipulation domain abstraction based off of \cite{He:RAL:2018}. 


\begin{definition}[Abstraction of a Manipulation Domain]
    \label{def:manip_domain_abstraction}
	An \emph{abstract manipulation domain} is a tuple: $G_{det}=(S, s_0, A_s, A_e, T, AP, L)$ where,
	\begin{itemize}
		\item $S$ is a finite set of states,
		\item $s_0 \in S$ is the initial state,
		\item $A_s$ is the finite set of system (robot) actions,
		\item $A_e$ is the finite set of environment (human) actions,
		\item $T : S \times (A_s \cup A_e) \mapsto S$ is the transition function,
		\item $AP$ is the set of task-related atomic propositions,
		\item $L : S \mapsto 2^{AP}$ is the labeling function that maps each state to a set of atomic propositions.
	\end{itemize}
\end{definition}

Consider the abstract manipulation domain depicted in \autoref{fig:abs_manip}. There are two agents, a robot and a human. Each agent can change the state of the world, albeit under some restrictions. For the robot, these restrictions follow typical PDDL pick-place domains \cite{pddl}. For example, the robot cannot pickup an object while it is supporting another object as in \autoref{fig:abs_manip}. For the human, we may have to include additional restrictions such as limiting the number of actions or the rate of interventions. On the other hand, we try to grant the human greater flexibility than the robot in our models. E.g., by allowing multiple human actions in quick succession or by giving the human priority over the robot 
% \autoref{fig:abs_manip}.\qh{I'm having difficulty understanding what this is trying to say. Isn't this a preliminary on manipulation domain?}


\begin{figure}[h]
    \centering
    \begin{subfigure}{0.25\columnwidth}
        \includegraphics[width=\textwidth]{figs/arch_locs}%
        % \caption{}
        \label{fig:toy_example_setup}
    \end{subfigure}
    \qquad \quad
    \begin{subfigure}{0.25\columnwidth}
        \includegraphics[width=\textwidth]{figs/arch_init}
        % \caption{}
        \label{fig:toy_example_initial}
    \end{subfigure}
    % \vspace{-1em}
    \caption{Manipulation domain: (left) the locations of interest, where the Else location ($Loc_1$) contains all objects not otherwise shown.
    (right) Initial state with red and yellow blocks at $Loc_2$ and $Loc_3$ and the blue block at $Loc_1$.}
    \label{fig:toy_example}
\vspace{-3 mm}
\end{figure}

Once we have a model of a manipulation domain, we next need some formal way to express properties of ``runs'' (executions) through this domain. As in \cite{wells2021probabilistic}, we use ``missing'' objects to denote objects in the ``Else'' region (see \autoref{fig:toy_example}).

\subsection{Linear Temporal Logic over Finite Traces}
While regular languages are typically specified using tools such as regular expressions, many tasks can be expressed more naturally in a temporal logic \cite{he2019efficient}. Linear temporal logic (\ltl) is a popular formalism used to specify temporal properties. Here, we are interested in \ltl interpreted over finite traces (\ltlf) \cite{de2013linear}.

\begin{definition}[\ltlf Syntax]
	An \ltlf formula is built from a set of atomic propositions $AP$ and is closed under the Boolean connectives as well as the ``next'' operator $X$ and the ``until'' operator $U$:
	\[
		\ltlfphi ::= \top   \mid   p   \mid   (\neg \ltlfphi)   \mid   (\ltlfphi_1 \wedge \ltlfphi_2)   \mid   (X \ltlfphi)  \mid  (\ltlfphi_1 U \ltlfphi_2)
	\]
	where $p \in AP$, $\top$ is ``true'', and $\neg$ and $\wedge$ are the ``negation'' and ``and'' operators in Boolean logic respectively.
\end{definition}

\noindent
The common temporal operators ``eventually'' ($F$) and ``globally'' ($G$) are defined as: $F \, \ltlfphi = \top \, U \, \ltlfphi$ and $G \, \ltlfphi = \neg F\, \neg \ltlfphi$.

%% Shorter version
The semantics of an \ltlf formula are defined over finite traces. A trace $\rho$ is a word in $(2^{AP})^*$ \cite{de2013linear}. Notation $\rho \models \ltlfphi$ denotes that trace $\rho \in (2^{AP})^*$ satisfies formula $\ltlfphi$. We say a run accomplishes $\ltlfphi$, if the trace associated with it $\rho \models \ltlfphi$.  For a more thorough treatment of \ltlf, see \cite{de2013linear, de2015synthesis}.

%%% Semantics one
% The semantics of \ltlf are defined as follows.

% \begin{definition}[\ltlf Semantics]
% 	The semantics of an \ltlf \hspace{0.5mm}formula are defined over finite traces. A trace $\rho$ is a word in $(2^{AP})^*$. Let $|\rho|$ denote the length of trace $\rho$ and $\rho[i]$ be the $i^{th}$ symbol of $\rho$. Further, $\rho, i \models \ltlfphi$ is read as: ``the $i^{th}$ step of trace $\rho$ is a model of $\ltlfphi$.'':
% 	\begin{itemize}
% 		\item $\rho , i \models \top;$
% 		\item $\rho , i \models p$ iff $p \in \rho[i];$
% 		\item $\rho , i \models \neg \ltlfphi$ iff $\rho, i \not \models \ltlfphi;$
% 		\item $\rho , i \models \ltlfphi_1 \wedge \ltlfphi_2$, iff, $\rho, i \models \ltlfphi_1$ and $\rho, i \models \ltlfphi_2;$
% 		\item $\rho , i \models X \ltlfphi$ iff $|\rho| > i+1$ and $\rho, i+1 \models \ltlfphi;$
% 		\item $\rho , i \models \ltlfphi_1 U \ltlfphi_2$ iff $\exists j$ s.t. $ i \leq j < |\rho|$ and $\rho, j \models \ltlfphi_2$ and $\forall k$, $i \leq k < j$, \; $\rho, k \models \ltlfphi_1$,
% 	\end{itemize}
% \end{definition}
% Finite trace $\rho$ satisfies $\ltlfphi$, denoted by $\rho \models \ltlfphi$, if $\rho, 0 \models \ltlfphi$.
% An $LTL_f$ formula $\ltlfphi$ defines a language $\mathcal{L}(\ltlfphi)$ over the alphabet $2^{AP}$. $\mathcal{L}(\ltlfphi)$ is a regular language, more specifically, $\mathcal{L(\ltlfphi)} = \{\rho \in (2^{AP})^* \mid \rho \models \ltlfphi\}$. 
% (recall that \ltlf has the expressivity of star-free regular languages).

\begin{example}[Example \ltlf specification]

Consider the \ltlf formula for constructing an arch from \autoref{fig:toy_example} with any two boxes as support and blue box on top. Thus, 
\begin{align*}
    \phi_\text{arch} = & F \left( p_{\text{box, support}_{1}} \land p_{\text{box, support}_{2}} \land p_\text{blue, top} \right) \land \\
    & \quad G \left( \neg(p_{\text{box, support}_{1}} \wedge p_{\text{box, support}_{2}}) \rightarrow \neg p_\text{blue, top} \right)
\end{align*}
% $$ F\ constructed \wedge G\ \neg\ safety\_violation $$
\label{ex:task_phi}
\end{example}

\subsection{Stochastic Models}

\ml{only introduce Stochastic Games.}

In prior work, human-robot interaction was modeled as a game with two strategic players \cite{he2019efficient}. While this has limitations, it works well for scenarios with no stochasticity and where stringent guarantees are required. 

% \begin{example}
%     For a purely strategic human with no stochasticity, the manipulation domain becomes a deterministic transition system.
%     \begin{figure}[h]
%         \vspace{0em}
%             \centering
%             \scalebox{0.94}{
%             \begin{tikzpicture}[auto,node distance=2.5cm,on grid,line width=0.4mm, initial/.style ={text=black,initial by arrow, initial left}, initial text=$ $]
%                 \tikzstyle{round}=[thick,draw=black,circle]
        
%                 % \node[state, label={\footnotesize $\emptyset$}] (s0) {$\langle 1,2,3 \rangle$};
%                 \node[state, initial, inner sep=1pt,minimum size=0pt] (s0) {\includegraphics[width=11mm]{figs/arch_init}};
%                 \node[state,inner sep=1pt,minimum size=0pt] (s1) [right=of s0] {\includegraphics[width=11mm]{figs/arch_grasped}};
%                 \node[state,inner sep=1pt,minimum size=0pt] (s2) [below=1cm of $(s0)!0.5!(s1)$] {\includegraphics[width=11mm]{figs/arch_other}};
%                 \node[state,accepting,inner sep=1pt,minimum size=0pt] (s3) [right=of s1] {\includegraphics[width=11mm]{figs/arch_final}};		
        
%                 \path[->] 	(s0) edge node {} (s1)
%                             (s0) edge node {} (s2);
%                 \path[->] 	(s1) edge [bend right=45] node [above] {} (s0)
%                             (s1) edge node [above] {} (s3);
%                 \path[->] 	(s2) edge [bend left=45] node [below] {} (s0);
%                 \path[->] 	(s3) edge [out=35,in=-55, looseness=4] node {} (s3);
%             \end{tikzpicture}
%             }
%             \caption{Example portion of abstraction of manipulation domain $G_{det}$ for a deterministic pick-and-place domain and task \autoref{ex:task_phi}. 
%             % The state-space is explained in \autoref{fig:toy_example}.
%             }
%             \label{fig:example_deterministic}
%     \end{figure}
% \end{example}

The 2-player game-based model is limiting in several ways. First, it reasons about the worst-case human behavior. Second, in order to win the game, we need to impose some limit on human interventions, e.g., $k$ human actions. Finally, it cannot express random human behavior or human behavior where we have observed a statistical pattern. To mitigate this issue, one line of work considers MDPs \cite{wells2021probabilistic}.

\subsubsection{Markov Decision Process}

MDPs allow us to express stochastic interactions efficiently but cannot accommodate two strategic agents. To build \mdpmanip from $G_{det}$, a combined probability distribution is built from the probabilities of human actions and of the effects of robot actions. Under this model, the human is not strategic, so each node in the MDP will have only one human action, i.e., ``\texttt{human-move}". An example of a simplified MDP with only the human action is shown in \autoref{fig:examplemdp}. Note that the human cannot manipulate objects in the robot's end-effector:

\begin{example}[MDP]
\begin{figure}[t!]
    \vspace{-1em}
    \label{ex:example_mdp_human}
        \centering
        \begin{tikzpicture}[auto,node distance=3cm,on grid,line width=0.4mm]
          \tikzstyle{round}=[thick,draw=black,circle]
    
            \node[state, rectangle, inner sep=1pt,minimum size=0pt] (s0) {\includegraphics[width=15mm]{figs/arch_init}};
            \node[state, rectangle, minimum size=0pt] (s6) [right=2.5cm of s0] {};
            \node[state, rectangle, accepting,inner sep=1pt,minimum size=0pt] (s1) [right=3.5cm of s6] {\includegraphics[width=15mm]{figs/arch_final}};
            \node[state, rectangle, inner sep=1pt,minimum size=0pt] (s2) [below=2.1cm of s6] {\includegraphics[width=15mm]{figs/arch_red_empty}};
            \node[state, rectangle, inner sep=1pt,minimum size=0pt] (s3) [below=2.1cm of s1] {\includegraphics[width=15mm]{figs/arch_empty_yellow}};		

            \node[state, rectangle, inner sep=1pt,minimum size=0pt] (s4) [above=2.1cm of s6] {\includegraphics[width=15mm]{figs/arch_another}};
            \node[state, rectangle, inner sep=1pt,minimum size=0pt] (s5) [above=2.1cm of s1] {\includegraphics[width=15mm]{figs/arch_yellow_red}};
            \node[draw=none,fill=none, right=1.5cm of s4] {\Large\dots};
            

            % MY version
            \path[->] 	%(s0) edge [in=180,out=0,pos=0.6] node [below] {\footnotesize \texttt{human-move}} (s6)
                        (s0) edge [in=180,out=0,pos=0.6] node [below] {} (s6)
                        (s6) edge [in=180,out=0,pos=0.8] node [above] {\footnotesize 0.15} (s1)
                        (s6) edge [in=55,out=0,pos=0.8] node [left=1mm] {\footnotesize 0.15} (s2)
                        (s6) edge [in=125,out=0,pos=0.8] node [left=1mm] {\footnotesize 0.15} (s3)
                        (s6) edge [in=35,out=45, pos=0.8] node [above=1mm] {\footnotesize 0.4} (s0)
                        (s6) edge [in=340,out=0,pos=1] node [above=0.25mm, right=1mm] {\footnotesize 0.03} (s4)
                        (s6) edge [in=195,out=0,pos=0.9] node [below=1mm] {\footnotesize 0.03} (s5);

            % %% Andrew's version
            % \node[state,inner sep=1pt,minimum size=0pt] (s0) {\includegraphics[width=13mm]{figs/arch_init}};
            % \node[state,accepting,inner sep=1pt,minimum size=0pt] (s1) [right=3.5cm of s0] {\includegraphics[width=13mm]{figs/arch_final}};
            % \node[state,inner sep=1pt,minimum size=0pt] (s2) [below=2.1cm of s0] {\includegraphics[width=13mm]{figs/arch_red_empty}};
            % \node[state,inner sep=1pt,minimum size=0pt] (s3) [below=2.1cm of s1] {\includegraphics[width=13mm]{figs/arch_empty_yellow}};		

            % \node[state,inner sep=1pt,minimum size=0pt] (s4) [above=2.1cm of s0] {\includegraphics[width=13mm]{figs/arch_another}};
            % \node[state,inner sep=1pt,minimum size=0pt] (s5) [above=2.1cm of s1] {\includegraphics[width=13mm]{figs/arch_yellow_red}};
            % \node[draw=none,fill=none, right=1.5cm of s4] {\Large\dots};
            % \node[state,minimum size=0pt] (s6) [right=1.5cm of s0] {};
            
            
            % \path[->] 	(s0) edge [in=180,out=0,pos=0.8] node [above] {\footnotesize 0.15} (s1)
            %             (s0) edge [in=55,out=0,pos=0.8] node [left=1mm] {\footnotesize 0.15} (s2)
            %             (s0) edge [in=125,out=0,pos=0.8] node [left=1mm] {\footnotesize 0.15} (s3)
            %             (s0) edge [in=12,out=2,loop,pos=0.9] node [above=1mm] {\footnotesize 0.4} ()
            %             (s0) edge [in=340,out=0,pos=1] node [above=0.25mm, right=1mm] {\footnotesize 0.03} (s4)
            %             (s0) edge [in=195,out=0,pos=0.9] node [below=1mm] {\footnotesize 0.03} (s5);
            
            % \path[->] 	(s1) edge node [above] {\footnotesize 0.9} (s0)
            %             (s1) edge [in=195,out=180,loop,pos=0.9] node [below=1mm] {\footnotesize 0.1} ()
            %             (s1) edge node [above,pos=0.7] {\footnotesize 0.9} (s3)
            %             (s1) edge [in=15,out=0,loop,pos=0.9] node [above=1mm] {\footnotesize 0.1} ();
            % \path[->] 	(s2) edge [bend right=30,pos=0.9] node [right=1mm] {\footnotesize 0.9} (s0)
            %             (s2) edge [in=110,out=100,loop,pos=0.9] node [left=0.25mm] {\footnotesize 0.1} ();
            %% loop for the action
            % \path pic[draw, angle radius=7mm,"\vphantom{g} \footnotesize{$a_1$}",angle eccentricity=1.3] {angle = s2--s0--s1};
            
        \end{tikzpicture}
        \caption{Example portion of an MDP encoding a human action. In the top row, the human has moved two and three blocks. In the remaining states, the human has moved one or no blocks.}
        \label{fig:examplemdp}
    \vspace{-1em}
\end{figure}

The human has probabilities for moving none, one or several of the blocks in \autoref{fig:examplemdp}. 
The robot can concurrently attempt to move blocks, deferring to the human in the case of conflict.
This results in a system with many possible transitions between states, where each transition can encode possibly several block motions. For example, in the top left, the robot may have tried to grasp the blue block, and has been overridden by the human's intervention.
% The human moved the yellow and then the red block in one transition.
\end{example}

We want to combine the expressivity of both models by considering two strategic players \em the human and the robot \em both with actions with stochastic outcomes. This enables us to reason over strategic agents whose actions can have stochastic outcomes.
% \qh{stochastic actions are different from actions with stochastic outcomes}

\subsubsection{Stochastic Games}
Now we formally define stochastic games.
\begin{definition}[Stochastic Game]
A stochastic game is a tuple $G = (S, s_0, A, T, C, AP, L)$ where $S, s_0, AP$ and $L$ are as in \autoref{def:manip_domain_abstraction} and:
\begin{itemize}
    % \item $S$ is a finite set of states
    % \item $s_0 \in S$ is the initial state
    \item $A$ is the finite set of actions
    \item $T: S \times A \times S \mapsto [0,1]$ is the probabilistic transition relation
    \item $C: S \mapsto \mathbb{N}$ designates which player controls the choice of action at each state
    % \item $AP$ is the finite set of atomic propositions
    % \item $L: S \mapsto 2^{AP}$ is the labeling function
\end{itemize}
We say $G$ is a two-player game when $C : S \mapsto \{0,1\}$.
% \km{Briefly comment about the Reward structure we use and note that we only use $\Pmax$ and $\Pmin$ specifications which do not reason over the rewards associated with states.}
\end{definition}

Intuitively, a stochastic game is similar to an MDP except that there are two (or more) independent strategic agents that take turns making choices.

\begin{definition}[Path through a Stochastic Game]
A path through a stochastic game is a finite sequence of states
$\lambda : s_0, ..., s_n$.
\end{definition}

\begin{definition}[Policy for a Stochastic Game]
A policy for a stochastic game is a function from a history of states and an action to a probability
$\sigma : \lambda \times A \mapsto [0,1]$
such that for any $\lambda$, $\sum_{act \in A} \sigma(\lambda, act) = 1$.
\end{definition}
 
For two player stochastic games with a reachability objective (as we have for \ltlf specifications), memoryless, deterministic policies suffice \cite{chen2013automatic}. In other words, each player need only consider the current state (memoryless) and need not make choices randomly (deterministic). Next we cover how to model manipulation as a stochastic game.

% \qh{A 2 player game (non-stochastic) does not preclude humans with stochastic actions. The optimal solution to most general sum games is usually a stochastic policy (I guess this is only true for non-fully observable games, but some clarification would be good). Up to here, there isn't a consistent message on why one needs stochastic games, other than the 'more expressive' probabilistic transitions. For e.g., example 2 can technically be modeled as a 2 player game because the stochasticity is not in the environment but in the strategy of the human. I think clarifying this would make the narrative clearer.}

% \km{Add Problem Formulation here!}


==> tikzfigures/ex_mdp_w_human.tex <==
\begin{figure}[t!]
    \vspace{-1em}
    \label{ex:example_mdp_human}
        \centering
        \begin{tikzpicture}[auto, node distance=3cm, on grid,line width=0.4mm]
          \tikzstyle{round}=[thick,draw=black,circle]
    
            \node[state, inner sep=1pt,minimum size=0pt] (s0) {\includegraphics[width=15mm]{figs/my_figures/arch_red_yellow_init.pdf}};
            % \node[state, minimum size=0pt] (s6) [right=2.5cm of s0] {};
            \node[state, inner sep=1pt,minimum size=0pt] (s1) [right=3.5cm of s6] {\includegraphics[width=15mm]{figs/my_figures/arch_red_yellow_blue_gripper.pdf}};
            \node[state, inner sep=1pt,minimum size=0pt] (s2) [below=2.1cm of s6] {\includegraphics[width=15mm]{figs/arch_red_empty}};
            \node[state, inner sep=1pt,minimum size=0pt] (s3) [below=2.1cm of s1] {\includegraphics[width=15mm]{figs/arch_empty_yellow}};		

            \node[state, inner sep=1pt,minimum size=0pt] (s4) [above=2.1cm of s6] {\includegraphics[width=15mm]{figs/arch_another}};
            \node[state, inner sep=1pt,minimum size=0pt] (s5) [above=2.1cm of s1] {\includegraphics[width=15mm]{figs/arch_yellow_red}};
            \node[draw=none,fill=none, right=1.5cm of s4] {\Large\dots};
            

            % MY version
            \path[->] 	(s0) edge [in=12,out=2, loop, pos=0.6] node [above] {\footnotesize 0.4} (s0)
                        (s0) edge [in=180,out=0,pos=0.8] node [above] {\footnotesize 0.15} (s1)
                        (s0) edge [in=55,out=0,pos=0.8] node [left=1mm] {\footnotesize 0.15} (s2)
                        (s0) edge [in=125,out=0,pos=0.8] node [left=1mm] {\footnotesize 0.15} (s3)
                        % (s0) edge [in=35,out=45, pos=0.8] node [above=1mm] {\footnotesize 0.4} (s0)
                        (s0) edge [in=340,out=0,pos=1] node [above=0.25mm, right=1mm] {\footnotesize 0.03} (s4)
                        (s0) edge [in=195,out=0,pos=0.9, looseness=1] node [below=1mm] {\footnotesize 0.03} (s5);
            
        \end{tikzpicture}
        \caption{Example portion of an MDP encoding human and robot actions. In the top row, the human has moved two and three blocks. In the remaining states, the human has moved one or no blocks.}
        \label{fig: examplemdp_karan}
    \vspace{-1em}
\end{figure}

==> title.tex <==
%auto-ignore
%\title{\LARGE \bf Probabilistic \ltlf Synthesis for Human-Robot Manipulation}
% \title{\LARGE \bf Probabilistic \ltlf Synthesis for Manipulation Domains}
\title{\LARGE \bf Stochastic Games for Interactive Manipulation Domains}

\author{Karan Muvvala$^{*1}$, Andrew M. Wells$^{*2}$, Morteza Lahijanian$^1$, Lydia E. Kavraki$^2$, and Moshe Y. Vardi$^2$ 
\thanks{This work was supported in part by NASA 80NSSC21K1031, NASA 80NSSC17K0162, NSF 1830549, and NSF RI 2008720.
% Work by AMW supported by NASA 80NSSC17K0162. 
Authors would also like to thank the authors of PRISM, especially Dr. Dave Parker for their excellent tool and for their help in modifying it to import stochastic games. }
\thanks{$^*$Equal contribution}
\thanks{$^1$Aerospace Eng. Sciences Dept. at the University of Colorado Boulder. \texttt{firstname.lastname@colorado.edu}}
\thanks{$^2$Computer Science Dept. at Rice University. Andrew Wells was a student at Rice University at the time this work was conducted.
\texttt{andrewmw94@gmail.com}, 
\texttt{\{kavraki,vardi\}@cs.rice.edu} }
}
